Covariance estimation using h-statistics in Monte Carlo and multilevel Monte Carlo methods

We present novel Monte Carlo (MC) and multilevel Monte Carlo (MLMC) methods to determine the unbiased covariance of random variables using h-statistics. The advantage of this procedure lies in the unbiased construction of the estimator's mean square error in a closed form. This is in contrast to conventional MC and MLMC covariance estimators, which are based on biased mean square errors defined solely by upper bounds, particularly within the MLMC. The numerical results of the algorithms are demonstrated by estimating the covariance of the stochastic response of a simple 1D stochastic elliptic PDE such as Poisson's model.

==> chapters/GMRF.tex <==
\subsection{Uncertainty modelling: Gaussian Markov random field}

Assuming that $\genSecTensor(\vek{x})$  represents an isotropic material, $\genSecTensor(\vek{x}) = \scalar(\vek{x}) \diag(\identitymatrix)$ is a diagonal matrix, where $\scalar(\vek{x})>0$ is a positive-definite scalar term. To incorporate the material uncertainty in spatial sense, the coefficient $\genSecTensor(\vek{x})$ is modelled as a tensor-valued SPD random field
\begin{equation}\label{Eq:Tmapping}
	\genSecTensor(\vek{x}, \event): \spatialdomain \times \samplespace\rightarrow\PosSymSecRankSpace
\end{equation}
on a probability space $(\samplespace,\sigmaalgebra,\probability)$. In other words, one may model
\begin{equation}\label{Eq:scalar,odel}
	\scalar(\vek{x}, \event): \spatialdomain \times \samplespace \rightarrow \mathbb{R}^+.
\end{equation}
Instead of modelling the previous equation, $\log(\scalar(\vek{x}, \event))$ can be modelled on $\mathbb{R}$ and take its exponential. Consequently, \feq{Eq:Tmapping} changes to:
\begin{equation}\label{Eq:Tmapping}
	\log(\genSecTensor(\vek{x}, \event)): \spatialdomain \times \samplespace\rightarrow\SymSecRankSpace,
\end{equation}
and taking $\exp(\log(\genSecTensor(\vek{x}, \event))) = \genSecTensor(\vek{x}, \event)$.
In this work, $\log(\scalar(\vek{x}, \event)):=\logscalar(\vek{x}, \event) $ from \feq{Eq:scalar,odel} is modelled as a Gaussian Markov random field (GMRF) with Mat\'{e}rn covariance structure \cite{lindgren_explicit_2011, bulthuis_implementation_2022} which can be attained as a solution to a stochastic PDE of the form:
\begin{equation}
	(\kappa-\Delta)^{\alpha/2} \logscalar(\vek{x}, \event) = \mathcal{W}(\vek{x}, \event).
\end{equation}
With an assumption of $\alpha=2$ and suitable boundary conditions (Neumann or Robin), one may peform spatial discretization using finite element method from  \feq{Eq:u_approx} as
\begin{equation}\label{}
	\logscalar(\vek{x}, \event)\approx\logscalar_h(\vek{x}, \event) = \sum_{j=1}^\nodes \logscalar_j(\event) \shapefunc_j(\vek{x}).
\end{equation}
%, where $\samplespace$ 
%represents the sample space containing all outcomes $\event\in\samplespace$, $\sigmaalgebra$ is the 
%$\sigma$-algebra of measurable subsets of $\samplespace$, and $\probability$ is 
%a probability measure.
One has to basically solve the linear system of equations
\begin{equation}\label{Eq:linGMRF}
	\vek{K} \vek{L}(\event) = \vek{M}^{1/2} \vek{\xi}(\event)
\end{equation}
to obtain the GMRF realisations of $\scalar(\vek{x}, \event)$. Here, solution vector is
$\vek{L}(\event) = [\zeta_j(\event)] \in \mathbb{R}^\nodes$ and the vector of independent standard Gaussian random variables is $\vek{\xi}(\event) = [\xi_j\sim\mathcal{N}(0, 1)] \in \mathbb{R}^\nodes$.  Furthermore, the entries of the matrices in the previous equation are given as:
\begin{equation}
	\begin{aligned}
		{M_{ij}} &= \langle \shapefunc_i, \shapefunc_j \rangle\\
		{G_{ij}} &= \langle \nabla \shapefunc_i, \nabla \shapefunc_j \rangle\\
		K_{ij} &= \kappa^2 M_{ij} + G_{ij}
	\end{aligned}
\end{equation}
To make $\vek{M}^{1/2} $ sparse in \feq{Eq:linGMRF}, the mass matrix $\vek{M}$ is approximated by a diagonal matrix of the form:
\begin{equation}
	\tilde{M_{ij}} =  \langle \shapefunc_i, 1 \rangle.
\end{equation}

==> chapters/old_text.tex <==
\section{Uncertainty Quantification}\label{UncertaintyQuantification}

Let be given physical system occupying domain $\mathcal{G}$ modelled by an equilibrium equation:
\begin{equation}\label{abs_main_eq}
A(q,\uu)=f, \quad \uu(0)=\uu_0,
\end{equation}
where $\uu \in \U$ describes the state of the system lying in a Hilbert space $\U$ (for the sake of simplicity), 
$A$ is a—possibly non-linear— operator modelling the physics of the system, and $f\in \U^*$ is some external influence (action / excitation / loading). Furthermore, we assume that the model depends on the parameter set $q \in \mathcal{Q}$ which is uncertain, and described in a tensor/matrix form. In other words, $q$ is modelled as a $n\times n$ dimensional positive-definite matrix-valued random variable/field with finite second order moments on a probability space $(\varOmega, \mathfrak{F}, \mathbb{P})$ where $\varOmega$ denotes the set of elementary events, $\mathfrak{F}$ is a $\sigma$-algebra of events, and $\mathbb{P}$ is a probability measure, i.e.
    \begin{equation}
	    q(x,\omega):\spatialdomain\times\samplespace\rightarrow\PosSymMatSpacenn.
    \end{equation}
Here
  \begin{equation}
        \PosSymMatSpacenn:=\{ \elastmatrix \in \Rn:\elastmatrix=\elastmatrix^T, \quad \vek{z}^T\elastmatrix \vek{z}>\vek{0}, \quad \forall \vek{z}\in\mathbb{R}^n\setminus\vek{0}\}.
    \end{equation}
%     \begin{equation}
% 	    q(x,\omega):\spatialdomain\times\samplespace\rightarrow\textcolor{red}{\PosSymNRankSpaceN}.
%     \end{equation}
% Here
%   \begin{equation}
%         \textcolor{red}{\PosSymNRankSpaceN:=\{ C \in (\Euclideanspace)^{\otimes m}:C=C^T, \  {z}\cdot C {z}>0, \ \forall {z}\in\mathbb{R}^n\setminus{0}\}.}
%     \end{equation}
Given uncertain $q$ the system  in \BRrefeq{abs_main_eq}
rewrites to the stochastic one:
\begin{equation}\label{basic_eq}
A(q(x,\omega),\uu(x,\omega))=f(x), \quad \uu(0)=u_0,
\end{equation}
which further is to be solved for $\uu(x,\omega) \in \U\otimes L_2(\varOmega, \mathfrak{F}, \mathbb{P})$. 
Note that in the previous equation the external influence $f$, as well as initial conditions $\uu_0$ can be also described as uncertain, and thus included in the parameter set. The theory presented further does not depend on this choice and is general enough to cover all of the mentioned cases. 

Given that the response of the model is uncertain, all its relevant information may be obtained via corresponding stochastic description.  Here we will focus on the $r$-th, $r\in\mathbb{N}$, central moment of $\uu \equiv \uu(x,\omega) $:
\begin{equation}\label{math_Exp}
		\mathbb{E}\left((\uu-\mathbb{E}(\uu))^r\right) = \int_\samplespace (\uu-\mathbb{E}(\uu))^r \probability(\text{d}\event)
\end{equation}
with ${\mu}(\uu):=\mathbb{E}(\uu)$ being the mean or the first raw moment and $\var(\uu):=\mathbb{E}\left((\uu-\mathbb{E}(\uu))^2\right) $ being the second central moment or the variance. The objective of this study is to determine these two moments after the appropriate discretization of the problem presented in \BRrefeq{basic_eq}.
		
Due to spatial and stochastic dependence, the solution $u$ in \BRrefeq{basic_eq} is first discretised in a spatial domain, i.e.~we search for the solution in a finite subspace $\U_\h\subset \U$.  After rewriting the problem in \BRrefeq{basic_eq} in a variational  form, the spatial discretisation $\uh(\omega)\in \U_\h$---$\h$ being the discretization parameter---can take the finite element form  on a sufficiently fine spatial grid $\mathcal{T}_h$ \footnote{Other types of discretization techniques can be considered as well}. The expectation functional in \BRrefeq{math_Exp}  then rewrites to:
\begin{equation}\label{math_Exp_h}
		\mathbb{E}((\uh-\mathbb{E}(\uh))^r) = \int_\samplespace (\uh-\mathbb{E}(\uh))^r \probability(\text{d}\event),
		\end{equation}
in which the exact solution $u$  is substituted by a semi-discretised solution $\uh \equiv \uh(\omega)$. 

Due to the complexity in integrating the above equations analytically, in this paper, the focus is on the sampling-based Monte Carlo (MC) estimators \cite{metropolis_monte_1949,fishman_monte_1996} that employ multi-level approximation of the finite element solution, also known as the multi-level Monte Carlo (MLMC) method \cite{Heinrich2001,giles2008,giles_2015}.  However, the multi-level version of the MC algorithm as employed in the literature is based on the classical absolute error estimates, and therefore the convergence of the algorithm strongly depends on the solution magnitude. 
In this article, we propose a new version of the algorithm in which the statistical relative error is proposed. The new estimate is taken to be scale-invariant meaning that the solution magnitude does not affect the algorithm convergence. 
		
\subsection{Monte Carlo estimation for the mean}\label{MC}

Let $\uhN:=\uh(\omega_i),\left\lbrace i=1,..,\N \right\rbrace$, be the fully-discretized solution of  \BRrefeq{basic_eq}, where $N$ is the sample size. Further, let each sample $\uh(\omega_i)$ come from the identical distribution as $\uh(\omega)$. For the unbiased estimate of the statistic of $g(\omega)$, we take symmetric function
% of $k$ variables and $n$ be a positive integer, $n\geq k$, then the average of values of $\phi$ over all points obtained from $(u_1,..,u_n)$ by extracting ordered subsets of $k$ $u$'s reads
%\begin{equation}
%\varphi^{[n]}=\varphi^{[n]}(u_1,..,u_n)
%\end{equation}
\begin{equation}\label{symmetric}
\mu^{\text{MC}}(g)=\frac{1}{\N}(g(\omega_1)+g(\omega_2)+...+g(\omega_N)),
\end{equation}
meaning that the estimate does not depend on the order in which observations were taken. The existence and uniqueness of such a choice are given in \cite{halmos1946}. By use of \BRrefeq{symmetric} one may formulate
%
%Then conditional expectation of .... introduce $\phi$ function that is symmetric and permutation independent. 
%\begin{eqnarray}
%add math here
%\end{eqnarray}
the \acrshort{mc} estimate of the mean $\mu(\uh)$ as
\begin{equation}
			\mu^{\text{MC}}(\uhN) := \frac{1}{\N}\sum_{i=1}^{\N}\uh(\event_i).
\end{equation}
%		According to the central limit theorem the MC mean is equal to the exact mean of the approximated solution:
%\begin{eqnarray}\label{samp_mean}
%			\mathbb{E}( \mu^{\text{MC}}(\stodisp) )&=&\mathbb{E}\left( \frac{1}{\N}\sum_{i=1}^{\N}\uh(x,\event_i)\right)=  \frac{1}{\N}\sum_{i=1}^{\N} \mathbb{E}(\uh(x,\event_i)) = \mathbb{E}(\uh(x,\event) ),
%		\end{eqnarray}
%whereas the MC variance of the mean reads:
%\begin{equation}\label{samp_var}
%			\text{Var}(\mu^{\text{MC}}(\stodisp)) = \frac{1}{\N} \text{Var}(\uh(x,\event)) .
%		\end{equation}
	Following this, the approximation error of the MC based mean estimate compared to the exact mean reads
%	\begin{eqnarray}
%			\mathbb{E}( \mu^{\text{MC}}(\stodisp) )&=&\mathbb{E}( \frac{1}{\N}\sum_{i=1}^{\N}\dispvectorApprox(x,\event_i)\nonumber \\ 
%			&=&  \frac{1}{\N}\sum_{i=1}^{\N} \mathbb{E}(\dispvectorApprox(x,\event_i)) \nonumber \\ 
%			&=& \mathbb{E}(\dispvectorApprox(x,\event) )
%		\end{eqnarray}
%		
%The error between the exact estimate and Monte Carlo approximation 
\begin{equation}
			 {\ee} = \mu^{\text{MC}}(\uhN) -\mathbb{E}(u),
		\end{equation}
which further can be rewritten as
		\begin{equation}\label{error}
			\ee = \mu^{\text{MC}}(\uhN) -\mathbb{E}(\uh) +\mathbb{E}(\uh) -\mathbb{E}(u).
		\end{equation}
		The first term in the previous equation is the sampling error $\ees:=\mu^{\text{MC}}(\uhN) -\mathbb{E}(\uh)$
%$\ees:=\mu^{\text{MC}}(\uhN) -\mathbb{E}(\uh(x,\event) )$ 
defined by a central limit theorem
\begin{equation}\label{Eq:varepsilons}
	\ees \sim \mathcal{N}\left(0, \frac{\var(\uh)}{\N} \right),
\end{equation} 
whereas the second term describes the spatial discretization error
$$\eed:=\mathbb{E}(\uh) -\mathbb{E}(u).$$
Thus, the \acrfull{mse} reads
\begin{equation}\label{Eq:MCerror1}
 {\ee_{\text{MSE}}}(\muMC(\uhN)) :=\mathbb{E}(({\ee})^2)= %\var(\mu^{\text{MC}}(\uhN)) + 
\frac{\var(\uh)}{\N}+
(\mathbb{E}(\uh) -\mathbb{E}(u))^2.
\end{equation}		

Our particular interest lies in reducing the sampling part of the error $\ees$ that depends on the variance of the solution, and thus on its magnitude. Hence, if each observation $\uh(\omega_i)$ is scaled by a parameter $c$ then the Monte Carlo error in \BRrefeq{Eq:MCerror1} will be affected in a square proportional manner, which is not suitable in practical applications. To overcome this issue, we first assume that variance $\var(\uh)$ is known and define the new error estimate with the help of t-statistic \cite{student_probable_1908,fisher_043_1925}:
		\begin{equation}\label{new_error}
			\e:= \frac{\ee}{\sqrt{\var(\uh)}} = \frac{\ee}{\std(\uh)},
		\end{equation}
		where $\std(\uh)$ is the standard deviation of the solution.
		Hence, the substitute for the sampling error in \BRrefeq{Eq:varepsilons} reads
		\begin{equation}\label{brsamp}
			\es   \sim \mathcal{N}\left(0, \frac{1}{\N}\right),
		\end{equation}
		and is dimensionless. In other words, the new type of error is scale-invariant under linear transformations of samples, which further makes $\es$ suitable candidate for the mean error estimator. 
		
By normalizing \BRrefeq{Eq:MCerror1} one obtains the squared error estimate 
	\begin{equation}\label{Eq:MCerror3}
			 {\e_{\text{MSE}}}(\muMC(\uhN)) :=\mathbb{E}(({\e})^2) = \frac{1}{N}+  \frac{(\mathbb{E}(u_{h})-\mathbb{E}(u))^2}{ \var(u_{h})},
		\end{equation}
 in which the second term represents the square of the new normalized discretization error $\ed:=\frac{\eed}{ \std(u_{h})} $. As in general the variance $\var(\uh)$ and hence the standard deviation $\std(\uh)$ are not known but estimated, the error defined in \BRrefeq{new_error} will take a slightly different form i.e.
	\begin{equation}\label{new_error1}
			 {\eMC_B}= \frac{\ee}{\sqrt{ \var^{\textrm{MC}}(\uhN)}} = \frac{\ee}{ \std^{\textrm{MC}}(\uhN)}.
			\end{equation}
 Here both variance $\var^\text{MC}(\uhN)$ and standard deviation $\std^{\text{MC}}(\uhN)$ estimators are determined by a \acrshort{mc} procedure with $N$ random draws. However, 
 in such a case the use of symmetric function as in \BRrefeq{symmetric} does not lead to an unbiased estimator any more. 
 
 Following \cite{halmos1946} from all unbiased estimators of variance, the only one that is symmetric and of minimum variance is given by 
  	\begin{equation}
 		\htwoMC(\uhN):= 
		 \frac{1}{N-1} \sum_{i=1}^N (\uh(\omega_i)-\mu^{\text{MC}}(\uh))^2. 
 	\end{equation}
% 	\begin{eqnarray}
%			\textrm{Var}^{\text{MC}} (\uhN)&=& \frac{N}{N-1} \frac{1}{N}\sum_{i=1}^N (\uh(x,\omega_i)-(\mu^{\text{MC}}(\uh)))^2 \nonumber\\
%			&=& \frac{1}{N-1} \sum_{i=1}^N (\uh(x,\omega_i)-\mu^{\text{MC}}(\uh))^2. 
%	\end{eqnarray}
This estimator is known as the second h-statistic and is further derived by 	\cite{dwyer1937} and implemented by \cite{Colin_Rose:2002}. Introducing the notion of power sum $S_r\equiv S_r(\uhN) := \sum_{i=1}^{\N}(\uh(\event_i))^r$, the second h-statistic can be also written as 
		\begin{equation}\label{arr}
			 \htwoMC(\uhN) = \frac{NS_2-S_1^2}{N(N-1)}.
		\end{equation}
%		Here, $\mathbb{E}(\dispvector)$ is the first raw moment of $\dispvector(x,\event)\equiv\dispvector$. The first term in the above equation denotes the statistical error of the estimator, and the second one represents the spatial discretization error. Following the law of large numbers, one may rewrite the sampling error as:
%		\begin{equation}\label{Eq:CLT}
%			\var(\mu^{\text{MC}}(\stodisp)) = \frac{\var(\dispvectorApprox)}{N}
%		\end{equation} 
%		where, 
%		\begin{equation}
%			{\var}(\dispvectorApprox) \approx {\text{V}^{\text{MC}}_1}(\stodisp) := \frac{1}{\N-1}\sum_{i=1}^{\N}(\dispvectorApprox(x,\event_i)-\mu^{\text{MC}}(\stodisp))^2.
%		\end{equation}
%		is the conventional expression of corrected sample variance, which is identical to \feq{Eq:MCerror1} viz. $\htwoMC(\stodisp) = {\text{V}_1}(\stodisp)$.
The substitution of \BRrefeq{arr} in \BRrefeq{new_error1} for $\varMC(u_{h,N})$ results in obtaining the complete error estimate for the mean:
	\begin{equation}\label{new_errorMEAN}
			{\eMC}= \frac{\ee}{\sqrt{\htwoMC(\uhN)}}.
			\end{equation}


\subsection{Monte Carlo estimation for the variance}\label{MCvar} 

The previously derived estimate in \BRrefeq{arr} is characterized by an approximation error given as
	\begin{equation}\label{Eq:MCvarerr1}
	 {\eev}=\htwoMC(\uhN)-\var(\uh)+\var(\uh)-\var(u),
	\end{equation}
	in which $\var(u)$ denotes the exact variance of the solution $u$.  Here
	 \begin{equation}
	 \eevs:=\htwoMC(\uhN)-\var(\uh)
	 \end{equation}
	 and
	 \begin{equation}
	 \eevd=\var(\uh)-\var(u)
	 \end{equation}
	 are the sampling and discretization errors, respectively. Hence, the MSE of the variance estimator reads:
		\begin{equation}\label{Eq:MCerror2}
		 {{\eev}_{\text{MSE}}}(\htwoMC(\uhN)) := \mathbb{E}(({\eev})^2)=\var(\htwoMC(\uhN)) +  ({\var}(\uh)-{\var}(\uu))^2.
		\end{equation}
	 Note that in contrast to the mean sampling error $\ees$ in \feq{Eq:varepsilons}, the variance sampling error $\eevs$ is not normally distributed anymore. The distribution type is application dependent and conditioned on the type of the distribution of $u$ we sample from. Despite this, the mean and variance of the variance estimate are known in the general case, and our attention will be paid to these.
 The variance of the second order statistic is derived by \cite{E_cho_2009} and reads
		\begin{equation}\label{Eq:varvar}
			\var( \htwoMC(\uhN)) := \frac{1}{N}\left( \mu_4(\uh) - \frac{\mu_2(\uh)^2(N-3)}{(N-1)}\right), 
		\end{equation}
	where $\mu_2(\uh)$ and $\mu_4(\uh)$ represent the second and fourth central population moments. 
%		and the above equation can equally be re-described as
%		\begin{equation}
%			\var(\htwoMC(\uhN)) \approx \frac{{\text{V}^{\text{MC}}_2}(\uhN)}{N}.
%		\end{equation}
%		It follows that,
%		\begin{equation}\label{Eq:V_2}
%			{\text{V}^{\text{MC}}_2}(\uhN) = \mu_4(\dispvectorApprox) - \frac{\mu_2(\dispvectorApprox)^2(N-3)}{(N-1)},
%		\end{equation}
The unbiased approximation of fourth central moment $\mu_4(\uh)$ is computed by the fourth h-statistic \cite{dwyer1937}:
\begin{multline}\label{Eq:mu_4}
\mu_4(\uh) \approx \text{h}_4^{\text{MC}}(\uhN) := \frac{1}{N(N - 1)(N - 2)(N - 3)} \bigg( -3S_1^4 + 6NS_1^2S_2 \\ + (9-6N)S_2^2 + (-4N^2+8N-12)S_1S_3
+ (N^3 - 2N^2 + 3N)S_4 \bigg),
\end{multline}
whereas the unbiased estimator of $\mu_2(\uh)^2$ is the polyache $\text{h}_{\left\lbrace 2,2\right\rbrace }$ according to \cite{tracy1974,Colin_Rose:2002}, given as
\begin{multline}\label{Eq:mu_2_2}
\mu_2(\uh)^2 \approx \text{h}_{\left\lbrace 2,2\right\rbrace}^{\text{MC}}(\uhN) := \frac{1}{N(N - 1)(N - 2)(N - 3)}\bigg(S_1^4 - 2NS_1^2S_2  \\+ (N^2 - 3N + 3)S_2^2 + (4N - 4)S_1S_3+ (- N^2 + N)S_4 \bigg).
\end{multline}
Therefore, by substituting \feqs{Eq:mu_4}{Eq:mu_2_2} in \feq{Eq:varvar}, one obtains the unbiased estimate $\var^{\text{MC}}(\htwoMC(\uhN))$ of $\var(\htwoMC(\uhN))$.
% Another way of deriving is explained in \cite{krumscheid_quantifying_2020}, where an ansatz is initially considered. Subsequently, the ansatz coefficients are determined by comparison between expectation of ansatz and \BRrefeq{Eq:varvar}.
Another way of deriving is explained in \cite{krumscheid_quantifying_2020}, where an ansatz is initially considered, whose coefficients are determined by comparison between expectation of ansatz and \BRrefeq{Eq:varvar}.

%	 \textcolor{yellow}{However, the error $\eevs$ is assumed to be of the order $\mathcal{O}(N^{-1})$ \cite{krumscheid_quantifying_2020}}.

For brevity, one may further rewrite \feq{Eq:varvar} as
\begin{equation}\label{Eq:V2N}
    \var( \htwoMC(\uhN)) := \frac{\Vtwo(\uh)}{N},
\end{equation}
where
\begin{equation}
    \Vtwo(\uh) := \mu_4(\uh) - \frac{\mu_2(\uh)^2(N-3)}{(N-1)}.
\end{equation}
 As in \feq{Eq:MCerror2}, only the term $\var(\htwoMC(\uhN))$ is needed,  the scale-invariant estimator will be defined only for this case. Hence, the new error estimate is given by normalizing \feq{Eq:MCvarerr1} in the form:
%\begin{equation}\label{Eq:MCerror2a}
%		e_v=\frac{\eev}{\sqrt{{\text{Var}_2^{\text{MC}}}(\uhN)  }}
%\end{equation}
\begin{equation}\label{Eq:MCerror2a}
\ev=\frac{\eev}{\sqrt{{\mathbb{V}_2}(\uh)}}.
\end{equation}
% 		in which 
%		\begin{equation}\label{Eq:V_2}
%			{\text{V}^{\text{MC}}}(\uhN) := \mu_4(\uh) - \frac{\mu_2(\uh)^2(N-3)}{(N-1)}.
%		\end{equation}
%		\begin{equation}\label{Eq:V_2}
%		{\text{Var}_2^{\text{MC}}}(\uhN) := N\varMC(\htwoMC(\uhN)).
%		\end{equation}
% 		\begin{equation}\label{Eq:V_2}
% 		{\Vtwo(\uh)} := N\var(\htwoMC(\uhN)).
% 		\end{equation}				
This further leads to
%	\begin{equation}\label{Eq:MCerror2b}
%		e_{\text{VMSE}}(\htwoMC(\uhN)) :=\mathbb{E}(\ev^2) = \frac{1}{N} + \frac{ ({\var}(\uh)-{\var}(\uh))^2}{{\text{Var}_2^{\text{MC}}}(\uhN)}.
%	\end{equation}

	\begin{equation}\label{Eq:MCerror2b}
		 {{\ev}_{\text{MSE}}}(\htwoMC(\uhN)) :=\mathbb{E}(({\ev})^2) = \frac{1}{N} + \frac{ ({\var}(\uh)-{\var}(\uu))^2}{{\Vtwo}(\uh)},
	\end{equation}	
	in which the first term is the scale-invariant sampling error $\evs$, and the second term represents the dimensionless discretization error $\evd:=\frac{({\eevd})^2}{{\Vtwo}(\uh)}$.	
The sample based unbiased estimation of quantity $\Vtwo(\uh)$ is therefore determined by
		\begin{equation}\label{Eq:Var_2}
			{\VtwoMC(\uhN)} := N\varMC(\htwoMC(\uhN)).
		\end{equation}

\feqsss{Eq:MCerror1}{Eq:MCerror3}{Eq:MCerror2}{Eq:MCerror2b}
%\feqs{Eq:MCerror1}{Eq:MCerror3}
%\BRrefeq{Eq:MCerror2} and \BRrefeq{Eq:MCerror2b} 
signify that to attain an overall higher level of accuracy, one requires a very fine resolution of finite element mesh-grid, and a very large number of \acrshort{mc} samples. This demands a tremendous amount of computational effort, making the algorithm practically unfeasible. Therefore, the desired moments are further estimated in a multi-level fashion following \cite{Heinrich2001,giles2008,giles_2015}. 
 
 \section{Multilevel Monte Carlo estimation for the mean}\label{MLMC}

Let $\left\lbrace \meshlevel=0,1,2...,\LL \right\rbrace$ be a generalised increasing sequence---in the context of decreasing the element size $h$---of nested mesh-grids $\mathcal{T}_\meshlevel$, a regular (non-degenerate) partition of  the computational domain $\mathcal{G}$ of the problem described in \BRrefeq{abs_main_eq}. Here $\meshlevel$ denotes the mesh level, and $\LL$ represents the finest mesh. Due to the linearity of the expectation operator, one may express the \acrshort{mlmc} (also denoted by ML) mean estimate of the mean $\mumu(\uhL)$ using a set of samples $\left\lbrace \Nl \right\rbrace:=\left\lbrace \N_0,\N_1,...,\N_L \right\rbrace$ as \cite{Heinrich2001}
		\begin{eqnarray}\label{Eq:meanMLMC}
			\muML(\uhLNL) &:=& \mu^{\text{MC}}(\uhONO) + \sum_{\meshlevel=1}^{\numofmesh}  \mu^{\text{MC}}(\uhlNl - \uhllNl) \nonumber\\
			&=& \sum_{\meshlevel=0}^{\numofmesh} \mu^{\text{MC}}(\YhlNl).
		\end{eqnarray}
		Here $\mu^{\text{MC}}(\uhONO)$ is the \acrshort{mc} estimator of mean $\mu(\uhO)$ on level $l=0$ using $N_0$ samples, and $\mu^{\text{MC}}(\uhlNl - \uhllNl)$ represents the approximation of mean $\mu(\uhlNl - \uhllNl)$ with $\meshlevel>0$ and $\Nl$ samples; $\mu^{\text{MC}}(\YhlNl)$ is the \acrshort{mc} estimator of $\mu(\Yhl)$ such that for $l=0$, $\YhONO = \uhONO$, otherwise $\YhlNl:=\uhlNl -\uhllNl$. Note that each term $\YhlNl, \ \meshlevel\ge{0}$ is sampled independently, whereas for $l>0$ the quantities $\uhlNl$ and $\uhllNl$ in $Y_{h_l,\Nl}$ are considered to be strongly correlated.
		
		As the mean estimate on the finest grid $\muML(\uhLNL)$ is obtained as the telescopic sum of the difference of \acrshort{mc} mean estimates on the coarser grids, the MSE corresponding to \BRrefeq{Eq:MCerror1} takes the form:
		 \begin{equation}\label{Eq:MLMCerror1}
			 {\eeML_{\text{MSE}}}(\muML(\uhLNL)) = \sum_{\meshlevel=0}^{\numofmesh} \frac{\var(\Yhl)}{\Nl}+(\mathbb{E}(\uhL)-\mathbb{E}(u))^2.
		\end{equation}
%		in which 
%		\begin{equation}
%			\text{Var}\left(\sum_{\meshlevel=0}^{\numofmesh} \mu^{\text{MC}}(\text{Y}_l)\right)=\sum_{\meshlevel=0}^{\numofmesh}\frac{\text{Var}(\text{Y}_l)}{\Nl}.
%		\end{equation}
	The above error consists of two terms, the variance of the estimator, given as $\eesML$ and the square of
spatial discretization error $\eedML:=\mathbb{E}(\uhL)-\mathbb{E}(u)$, similar to the MC error estimate. 
%To then achieve an overall error, the first term in \feq{Eq:MLMCerrornew3} is chosen to be less than $\frac{e_{\text{MLMSE}}}{2}$.
As the variance of the estimator  is not scale-invariant, we suggest the new MSE estimate following \BRrefeq{new_error}:
% 		\begin{equation}\label{Eq:MLMCerrornew1}
%			e_{\text{MLMSE}}(\muML(\uhLNL)) = \frac{\var\left(\sum_{\meshlevel=0}^{\numofmesh} \mu^{\text{MC}}({Y}_l)\right)}{\var(\uhLNL)}+\frac{(\mathbb{E}(\uhL)-\mathbb{E}(u))^2}{\var(\uhLNL)}
%		\end{equation}
 		\begin{equation}\label{Eq:MLMCerrornew2}
			 {\eML_{\text{MSE}}}(\muML(\uhLNL)) = \frac{1}{\var(\uhL)}\left(\sum_{\meshlevel=0}^{\numofmesh} \frac{\var(\Yhl)}{\Nl}\right) +\frac{(\mathbb{E}(\uhL)-\mathbb{E}(u))^2}{\var(\uhL)}.
		\end{equation}	
%in which $\varMC(\uhLNLL)$ is the MC variance estimator of $\var(\uhL)$. However, the normalization term $\varMC(\uhLNLL)$ in the previous equation is generally not known. Hence, under the assumption that for any value of $l$ and fixed $\Nl$, $\varMC(\uhlNl)$ will be approximately constant \cite{Cliffe2011}, one may substitute $\varMC(\uhLNLL)$ with $\varMC(\uhONO)$. This transforms \feq{Eq:MLMCerrornew2} to
% 		By defining the MC variance estimate of $\var(\Yhl):=\var(\uhl-\uhll)$ via $\varMC(\YhlNl)$, one may rewrite
% 		the above equation as
% 		 \begin{equation}\label{Eq:MLMCerror2}
% 			\eeML_{\text{MSE}}(\muML(\uhLNL)) = \sum_{\meshlevel=0}^{\numofmesh} \frac{\varMC(\YhlNl)}{\Nl}+(\mathbb{E}(\uhL)-\mathbb{E}(u))^2.
% 		\end{equation}
However, the normalization term $\var(\uhL)$ in the previous equation is generally not known. Hence, under the assumption that for any value of $l$, $\var(\uhl)$ will be approximately constant \cite{giles_2015,Cliffe2011}, one may substitute $\var(\uhL)$ with $\var(\uhO)$. Under the consideration that $\htwoMC(\uhONO)$ is the MC estimator of $\var(\uhO)$, and by defining the MC variance estimate of $\var(\Yhl):=\var(\uhl-\uhll)$ via $\htwoMC(\YhlNl)$, \feq{Eq:MLMCerrornew2} therefore transforms to	
% 		\begin{equation}\label{Eq:MLMCerrornew3}
% 		\eML_{\text{MSE}}(\muML(\uhLNL)) =\left(  \frac{1}{N_0}+\frac{1}{\varMC(\uhONO)}\left( \sum_{\meshlevel=1}^{\numofmesh} \frac{\varMC(\YhlNl)}{\Nl}\right)\right)  +\frac{(\mathbb{E}(\uhL)-\mathbb{E}(u))^2}{\varMC(\uhONO)},
% 		\end{equation}
 		\begin{equation}\label{Eq:MLMCerrornew3}
			 {\eMCMSE}(\muML(\uhLNL)) = \frac{1}{\htwoMC(\uhONO)}\left( \sum_{\meshlevel=0}^{\numofmesh} \frac{\htwoMC(\YhlNl)}{\Nl}\right)  +\frac{(\mathbb{E}(\uhL)-\mathbb{E}(u))^2}{\htwoMC(\uhONO)}.
		\end{equation}
% 		where $\varMC(\uhONO)$ represents MC variance estimation of $\var(\uhO)$.	
 		The first entity here stands for the scale-invariant multi-level sampling error $\esML$, whereas the second term defines the dimensionless discretization error $\edML$.  {Therefore, to attain an overall MSE of $\epssq$, it is adequate to satisfy the conditions such as $\esML<\epssqtwo$ and $\edML<\epssqtwo$.} 
%$\edML:=\frac{{\eedML}^2}{\varMC(\uhONO)}$.

If $\costlevel\equiv\mathcal{C}(\YhlNl)$ is the computational cost of determining single \acrshort{mc} sample of $\YhlNl$, then the overall cost of the estimator $\muML(\uhLNL)$ is given as $\mathcal{C}(\muML(\uhLNL)):=\sum_{\meshlevel=0}^{\LL}\Nl\costlevel$.
%In this study, the focus is only on satisfying the sampling error $\esML$. However, the deterministic error $\edML$ is assumed to be already achieved, meaning that the optimal level $\LL$ is known.
%In this study, as the deterministic error $\edML$ is assumed to be already achieved, meaning that the optimal level $\LL$ is known, the focus is only on satisfying the sampling error $\esML$.
In this study, the focus is only on satisfying the condition of sampling error under the assumption that the optimal level $\LL$ is known. The optimum number of samples $\Nl$ on each level $l$ is evaluated by solving a constrained optimization problem. That is, for a given error $\epssqtwo$, the cost function
\begin{equation}\label{Eq:costfn}
\costfunction = \text{arg} \min\limits_{\optSam}  \sum_{\meshlevel=0}^{\LL} \left(  \optSam\costlevel +  \Lagrange \frac{\htwoMC(\YhlNl)}{\htwoMC(\uhONO) \Nl}\right)
\end{equation} 	
is minimized. Thereby the optimal samples $\Nl$ are calculated as
\begin{equation}\label{eq:\Nl}
\optSam = \Lagrange\left({\frac{\htwoMC(\YhlNl)}{\htwoMC(\uhONO) \costlevel}}\right)^{\frac{1}{2}},
\end{equation}
where $\Lagrange$ is the Lagrange multiplier, determined by
\begin{equation}\label{Eq:tau}
\Lagrange \ge { {\frac{2}{\epssq}}}\sum_{\meshlevel=0}^{\numofmesh}\left( \frac{{\htwoMC(\YhlNl)\costlevel}}{\htwoMC(\uhONO)}\right) ^{\frac{1}{2}}.
\end{equation} 	

Let us consider the positive constants $c_1,c_2,c_3,\convorder,\convbeta,\convgamma$, given that $\convorder\ge\frac{1}{2}\text{min}(\convbeta,\convgamma)$ and assume that the following error bounds  \cite{giles2008,giles_2015} 		
\begin{equation}\label{eq:errormean1}
\begin{split}
|\mathbb{E}(\uhl)-\mathbb{E}(\uu)| &\le \constantofpropnew \h_\meshlevel^{\convorder},\\
\htwoMC(\YhlNl) &\le \conspropVar \h_\meshlevel^{\convbeta}, \\
\costlevel &\le \conspropTime \h_\meshlevel^{-\convgamma},
\end{split}
\end{equation}
hold. Then, there exists another positive constant $c_4$, such that for any $0<\epsilon<e^{-1}$, the \acrshort{mlmc} error estimator satisfies $\eMCMSE(\muML(\uhLNL))<\epssq$, and the total computational cost is bound by
\begin{equation}\label{Eq:costcomplex}
\mathcal{C}(\muML(\uhLNL))\le 
\begin{cases}
c_4\epsilon^{-2}, \quad &\convbeta>\convgamma,\\
c_4\epsilon^{-2(\log\epsilon)^2}, \quad &\convbeta=\convgamma,\\
c_4\epsilon^{-2-(\convgamma-\convbeta)/\convorder}, \quad &\convbeta<\convgamma.
\end{cases}
\end{equation}


%\begin{equation}\label{eq:errormean2}
%\begin{split}
%\frac{|\mathbb{E}({u}_{h_l})-\mathbb{E}(u)|}{\var(\uhONO)} &\le \constantofpropnew h_l^{\convorder},\\
%\frac{\var(Y_l)}{\var(\uhONO)} &\le \conspropVar h_l^{\convbeta}, \\
%\mathcal{C}(Y_l) &\le \conspropTime h_l^{-\convgamma},
%\end{split}
%\end{equation}
%
% Note that the second term is exactly
%the same as before in (2), and so it is sufficient to choose
%M = ML  ε−1/α again. To then achieve an overall RMSE
%of ε, the first term in (8) has to be less than ε2/2 as well.
%		\begin{equation}
%			\text{Var}\left(\sum_{\meshlevel=0}^{\numofmesh} \mu^{\text{MC}}(\text{Y}_l)\right)\approx \sum_{\meshlevel=0}^{\numofmesh}\frac{\text{V}^{\text{MC}}_1(\text{Y}_l)}{\Nl} ????????????????
%		\end{equation}
%		
\subsection{Multilevel Monte Carlo estimation for the variance}\label{MLMCvar}
		To enhance the characterization of probabilistic system response, this paper also focuses on defining the \acrshort{mlmc} estimator of $\var(\uhL)$ using h-statistics \cite{krumscheid_quantifying_2020}, expressed in the form:
		\begin{eqnarray}\label{Eq:varMLMC}
			\htwoML(\uhLNL) &:=& \htwoMC(\uhONO) + \sum_{\meshlevel=1}^{\LL}\left( \htwoMC(\uhlNl) - \htwoMC(\uhllNl) \right).
		\end{eqnarray}
		Here $\htwoMC(\uhONO)$ is the MC estimator of $\var(\uhO)$ with $\N_0$ samples; $\htwoMC(\uhlNl)$ and $\htwoMC(\uhllNl)$ represent the MC estimation of $\var(\uhl)$ and $\var(\uhll)$ using $\Nl$ samples, respectively.
		For simplification, we introduce:
		\begin{equation}\label{Eq:Zl}
		\Zl= 
		\begin{cases}
		\htwoMC(\uhONO),\quad &\meshlevel=0,\\
		\htwoMC(\uhlNl) - \htwoMC(\uhllNl),\quad &\meshlevel>0.
		\end{cases}
		\end{equation}
		Note that, for $\meshlevel>0$, $\uhlNl$ and $\uhllNl$ in $\Zl$ are determined using the same random seed.
		Thus, the expansion in \feq{Eq:varMLMC} is rewritten as 
		\begin{equation}
			\htwoML(\uhLNL)	= \sum_{\meshlevel=0}^{\numofmesh} \Zl.
		\end{equation}
%		here, when $l=0$, ${Z}_0 = \htwoMC(\uhONO)$, else $\Zl=\htwoMC(\uhlNl) - \htwoMC(\uhllNl)$. 
		In correspondence to \feq{Eq:MCerror2}, the MSE of the estimator $\htwoML(\uhLNL)$ takes the form:
		\begin{equation}\label{Eq:MLMCerrorvar}
			 {{\eevML}_{\text{MSE}}}(\htwoML(\uhLNL)) = \var\left(\htwoML(\uhLNL) \right)  +  ({\var}(\uhL)-{\var}(\uu))^2.
		\end{equation}
		Under further consideration that the quantity $\Zl$, for $\meshlevel\ge0$, are sampled independently,
		one may express the first term in the above equation as
		\begin{equation}\label{Eq:sampleerror}
			\var\left(\htwoML(\uhLNL) \right)  = \sum_{\meshlevel=0}^{\numofmesh} \var(\Zl),
		\end{equation}
		in which the variance $\var(\Zl)$ is further defined---simiar to \feq{Eq:V2N}---by ${\Vltwo}/{\Nl}$.
		Therefore, \feq{Eq:MLMCerrorvar} is reformulated to
		\begin{equation}\label{Eq:MLMCerrorvar1}
			{\eevML}_{\text{MSE}}(\text{h}_2^{\text{ML}}(\uhLNL)) = \sum_{\meshlevel=0}^{\numofmesh} \frac{\Vltwo}{\Nl}  +  ({\var}(\uhL)-{\var}(\uu))^2.
		\end{equation}
%		\begin{equation}\label{Eq:MLMCerrorvar1}
%			{\eevML}_{\text{MSE}}(\text{h}_2^{\text{ML}}(\uhLNL)) = \var\left( \sum_{\meshlevel=0}^{\numofmesh} \Zl\right)  +  ({\var}(\uhL)-{\var}(\uh))^2.
%		\end{equation}		
%		\begin{equation}
%		\var(\Zl) = -\frac{(\Nl - 2)\mu_{1,1}^2}{(\Nl-1)\Nl}+\frac{\mu_{0,2}\mu_{2,0}}{(\Nl-1)\Nl}+\frac{\mu_{2,2}}{\Nl}, \quad \meshlevel=0,1,2...,\LL
%		\end{equation}

		Following the notion of power sum $S_r$ defined in \fsec{MC}, here we introduce the bivariate power sum \cite{Colin_Rose:2002,krumscheid_quantifying_2020}
		\begin{equation}
		S_l^{a,b} := \sum_{i=1}^{\N} {X_{\h_l}^+(\event_i)}^a {X_{\h_l}^-(\event_i)}^b,
		\end{equation}	
		where 
		$ X_{\h_l}^+(\event_i)_{i=1,...,\Nl} := X_{\h_l,\Nl}^+ = \uhlNl + \uhllNl $
		and
		$ X_{\h_l}^-(\event_i)_{i=1,...,\Nl} := X_{\h_l,\Nl}^- = \uhlNl - \uhllNl $.			
		Subsequently, the unbiased MC estimation of the quantity $\Vltwo$ in \feq{Eq:sampleerror} reads:
		\begin{equation}
		\begin{split}
			{\VltwoMC} = \frac{1}{(\Nl-3)(\Nl-2)(\Nl-1)^2 \Nl}\Big( \Nl\big( ( -\Nl^2+\Nl+2){(S_l^{1,1}})^2  \\
			+(\Nl-1)^2 (\Nl S_l^{2,2}-2S_l^{1,0}S_l^{1,2}) + (\Nl-1)S_l^{0,2}(({S_l^{1,0}})^2-S_l^{2,0})\big) \\
			+ ({S_l^{0,1}})^2\big((6-4\Nl)({S_l^{1,0}})^2 + (\Nl-1)\Nl S_l^{2,0}\big)- \\ 
			2\Nl S_l^{0,1}\big((\Nl-1)^2 S_l^{2,1}+(5-3\Nl)S_l^{1,0}S_l^{1,1}\big) \Big).
		\end{split}	
		\end{equation}		
%		\begin{equation}\label{}
%			\Vltwo := \Nl \var(\Zl), \quad \meshlevel=0,1,2...,\LL
%		\end{equation}						
%		\begin{equation}
%			 S^{a,b}(X_{\h_l,\Nl}^+,X_{\h_l,\Nl}^-) := \sum_{i=1}^{\N} {X_{\h_l}^+(x,\event_i)}^a {X_{\h_l}^-(x,\event_i)}^b
%		\end{equation}
		Analogous to \feq{Eq:MCerror1}, the MSE in \feq{Eq:MLMCerrorvar1} is split into statistical error $\eevsML$---which is of the order $\mathcal{O}(\Nl^{-1})$---and square of deterministic bias $\eevdML:={\var}(\uhL)-{\var}(\uh)$. As described in \feq{Eq:Var_2}, the MSE ${\eevML}_{\text{MSE}}$ is transformed to a scale-invariant version ${\evML}_{\text{MSE}}$ by considering $\Vtwo(\uhL)$ as the normalization constant. However, we make an assumption that the value of $\Vtwo(\uhl)$ stays approximately close for all values of $\meshlevel$, i.e., $\Vtwo(\uhL) \approx \Vtwo(\uhO)$. If $\VtwoMC(\uhONO)$ is the MC estimator of  $\Vtwo(\uhO)$, then the new normalized MSE is given in the form:
%		\begin{equation}\label{Eq:MLMCerrorvar2}
%			{\evML}_{\text{MSE}}(\text{h}_2^{\text{ML}}(\uhLNL)) = \frac{1}{\VtwoMC(\uhLNL)} \left( \sum_{\meshlevel=0}^{\numofmesh} \frac{\VltwoMC}{\Nl} \right)  +  ({\var}(\uhL)-{\var}(\uh))^2.
%		\end{equation}
		\begin{equation}\label{Eq:MLMCerrorvar3}
			 {\evMCMSE}(\text{h}_2^{\text{ML}}(\uhLNL)) = \frac{1}{\VtwoMC(\uhONO)} \left( \sum_{\meshlevel=0}^{\numofmesh} \frac{\VltwoMC}{\Nl} \right)  +  \frac{({\var}(\uhL)-{\var}(\uu))^2}{\VtwoMC(\uhONO)}.
		\end{equation}			
		Here the first term defines the scale-invariant sampling error $\evsML$, and the second term is the normalized deterministic error $\evdML$. 
		 { Thus, the accomplishment of total MSE $\epsvsq$ is justified by ensuring that both errors $\evsML$ and $\evdML$ are lesser than $\epsvsqtwo$.}
		
		As the focus of this article is only on satisfying the constraint $\evsML<\epsvsqtwo$, one may determine the samples $\Nl$ analogous to \feeqs{Eq:costfn}{Eq:tau} as		
%		\begin{equation}
%		\costfunction = \text{arg} \min\limits_{\optSam}  \sum_{\meshlevel=0}^{\numofmesh} \left(  \optSam\costlevel +  \Lagrange_v \frac{\VltwoMC}{\VtwoMC(\uhONO) \Nl}\right)
%		\end{equation} 	
%		is minimized. Thereby the optimal samples $\Nl$ are calculated as
		\begin{equation}\label{}
		\optSam = { {\frac{2}{\epsvsq}}}\sum_{\meshlevel=0}^{\numofmesh}\left( \frac{{\VltwoMC\costlevel}}{\VtwoMC(\uhONO)}\right) ^{\frac{1}{2}}\left({\frac{\VltwoMC}{\VtwoMC(\uhONO) \costlevel}}\right)^{\frac{1}{2}}.
		\end{equation}
%		Here $\Lagrange$ is the Lagrange multiplier, determined as
%		\begin{equation}
%		\Lagrange_v \ge {\frac{1}{\evsML}}\sum_{\meshlevel=0}^{\numofmesh}\left( \frac{{\VltwoMC\costlevel}}{\VtwoMC(\uhONO)}\right) ^{\frac{1}{2}}.
%		\end{equation} 
		Note that, here $\costlevel$ is the computational cost of evaluating one MC sample of $\uhlNl$ and $\uhllNl$ in the difference term $\Zl$, which is equivalent to determining the cost of $\YhlNl$ in \feq{Eq:costfn}.
		
		Let us introduce the positive constants $c_5,c_6,\convorderv,\convbetav$, such that $\convorderv\ge\frac{1}{2}\text{min}(\convbetav,\convgamma)$ and the error bounds  \cite{krumscheid_quantifying_2020}
		\begin{equation}\label{eq:errorvar1}
		\begin{split}
		|\var({u}_{h_l})-\var(u)| &\le c_5 h_l^{\convorderv},\\
		\VltwoMC &\le c_6 h_l^{\convbetav}, \\
		\mathcal{C}_l &\le \conspropTime h_l^{-\convgamma},
		\end{split}
		\end{equation} 	
		are satisfied. Thus, one may state that, for any $0<\epsilon_v<e^{-1}$, the total MSE is bound by
		$\evMCMSE(\htwoML(\uhLNL))<\epsvsq$ with a computational cost
		\begin{equation}\label{Eq:costcomplex2}
		\mathcal{C}(\htwoML(\uhLNL))\le 
		\begin{cases}
		c_7\epsilon_v^{-2}, \quad &\convbetav>\convgamma,\\
		c_7\epsilon_v^{-2(\log\epsilon_v)^2}, \quad &\convbetav=\convgamma,\\
		c_7\epsilon_v^{-2-(\convgamma-\convbetav)/\convorderv}, \quad &\convbetav<\convgamma.
		\end{cases}
		\end{equation}	
		Here $c_7>0$ is a constant. 








%
%
%yes, there are ... too many ! See Mann Whitney Wilcoxon as a starter
%but non normality is not always sooo bad when using t-test because the important thing is the normality of the mean
%this normality of the mean is guaranteed if the sample is drawn from a normal law ; that's the easy part
%now, CLT also tells you that the distribution of the mean will be asymptotically normal (if you can assume finite first two moments ... with refinements on the convergence from Barry-Esseen bound if required ...) so using the t-test in the case of non-normal samples boils down to deciding whether you are or not in this asymptotic regime ; there are three main ingredients here, the size of the sample (your sample must be large), the "fattiness" of the distribution of your sample (the fatter the tail, the slower the convergence to the asymptotic regime) and the confidence level (the higher the confidence level, the higher the size of your sample since you are probing further into the tail of the distribution of the mean)
%
%. In case of the t-test you are interested in the expected values (or the expected difference). The test is not exact when the distribution (of the residuals) is not normal, but if this is the case (no normal residuals) the t-test is still the only test we have that adresses the expected difference.
%According to the central limit theorem, the distribution of sample mean values tends to follow the normal distribution regardless of the population distribution if the sample size is large enough [2]. For this reason, there are some books which suggest that if the sample size per group is large enough, the t-test can be applied without the normality test. Strictly speaking, this is not true. Although the central limit theorem guarantees the normal distribution of the sample mean values, it does not guarantee the normal distribution of samples in the population. The purpose of the t-test is to compare certain characteristics representing groups, and the mean values become representative when the population has a normal distribution. This is the reason why satisfaction of the normality assumption is essential in the t-test. Therefore, even if the sample size is sufficient, it is recommended that the results of the normality test be checked first. Wellknown methods of normality testing include the Shapiro–Wilks test and the Kolmogorov–Smirnov test. Hence, can the t-test be conducted with a very small sample size (e.g., 3) if the normality test is satisfied?

%    As the input uncertainties are modelled as a matrix-valued random field $\CRF$ and the determination of solution $\dispvectorApprox(x,\event)$ on a sufficiently fine spatial grid, this results in a high dimensional stochastic problem. In this work, the goal is to find the statistical moments, in particular, mean and variance of the stochastic response $\dispvectorApprox(x,\event)$ with computational efficiency. For this type of problem, it is well known that the non-sampling techniques often suffer from curse of dimensionality. Therefore, this paper emphasizes on implementing sampling based methods such as Monte Carlo (\acrshort{mc}) and \acrfull{mlmc}. First, the overview of Monte Carlo estimation is given in \fsec{MC}, and \fsec{MLMC} explains the \acrshort{mlmc} mean and variance estimators.

%    \subsection{Monte Carlo estimation}\label{MC}
%
%		In general, for $r\in\mathbb{N}$, the $r$-th central moment of $\dispvectorApprox(x,\event)\equiv\dispvectorApprox$ is defined as
%
%
%		Given, i.i.d samples $[\elastmatrix(x,\event_i)]_{i=1}^{N}$ of random elasticity matrix, where $\N$ is the sample size, one can compute probabilistic finite element solution  $\stodisp:=[\dispvectorApprox(x,\event_i)]_{i=1}^{N}$. Following this, the unbiased sample mean is given by:
%		\begin{equation}
%			{\mu}(\dispvectorApprox) \approx \mu^{\text{MC}}(\stodisp) := \frac{1}{\N}\sum_{i=1}^{\N}\dispvectorApprox(x,\event_i).
%		\end{equation}

		



==> chapters/problem.tex <==
\section{Problem description}

\begin{equation}
	\mathcal{L}(\kappa, \uu) = f
\end{equation}
%
%probability space $(\samplespace,\sigmaalgebra,\probability)$
%
%\begin{equation}\label{Eq:scalar,odel}
%	\kappa(\event): \samplespace \rightarrow \mathbb{R}^+.
%\end{equation}






==> chapters/stochastic_heat_eqn.tex <==
%\subsection{Stochastic setting of the problem}

Let's consider, for instance, stochastic Poisson equation
\begin{equation}\label{Eq:stochastic-thm}
	\begin{aligned}
		-\nabla\cdot(\genSecTensor(\vek{x}, \event) \nabla \uu(\vek{x},\event)) &= \heatsource(\vek{x})\quad \forall \vek{x}\in\spatialdomain, \event\in\samplespace, \\
		\uu(\vek{x},\event)) &= {\uu}_0,  \quad \forall \vek{x}
		\in \Gamma_D, \\
		\genSecTensor(\vek{x}, \event) \nabla \uu(\vek{x},\event))\cdot\vek{n}(\vek{x}) &= {g}(\vek{x}), \quad \forall \vek{x} \in \Gamma_N,
	\end{aligned}
\end{equation}
%where, only the diffusion coefficient $\genSecTensor$ is modelled as a random field
%\begin{equation}\label{Eq:Tmapping}
%	\genSecTensor(\vek{x}, \event): \spatialdomain \times \samplespace\rightarrow\PosSymSecRankSpace.
%\end{equation}
%%Weak formulation under uncertainty:
%%\begin{equation}\label{Eq:Sto_Weakform}
%%	a(\uu(\vek{x},\event),\testfunction(\vek{x},\event)) = l(\testfunction(\vek{x},\event)), \; \forall\testfunction(\vek{x},\event) \in \solspace\otimes \stospace,
%%\end{equation}
%After performing weak formulation, the stochastic finite element solution reads
%\begin{equation}\label{Eq:Sto_u_approx}
%	\uh(\vek{x},\event) = \sum_{j=1}^{\nodes} \solcoeff^h_j(\event) \shapefunc_j(\vek{x}).
%\end{equation}
%Consequently, one obtains linear system of equations
%\begin{equation}\label{}
%	\stiffnessmatrix(\event)\solvect^h(\event)=\vek{b},
%\end{equation}
%in which, $\solvect^h(\event) = [u^h_1(\event), u^h_2(\event),....,u^h_M(\event)]^T  \in \mathbb{R}^\nodes $ is the stochastic nodal solution vector.  
%with
%\begin{equation}
%	\stiffnessmatrix(\event) = [\stiffnessmatrixele_{ij}(\event)],\  \stiffnessmatrixele_{ij}(\event) = \int_\spatialdomain \nabla \shapefunc_i(\vek{x})^T \cdot \genSecTensor(\vek{x}, \event) \cdot \nabla \shapefunc_j(\vek{x}) \di\spatialdomain,
%\end{equation}

==> chapters/text.tex <==

%Objective: Why estimate covariance of solution?
%Fast estimation of covariance matrix of, let's say, stochastic finite element solution for faster data assimilation/filtering; especially for high dimensional stochastic problems.
%

\section{Motivation} 

Solving stochastic differential equations with high-dimensional random input parameters--due to the so-called curse of dimensionality issue---with computational efficiency is a major challenge in uncertainty quantification (UQ). In order to solve such stochastic problems, the Monte Carlo method (MC) has long been considered the gold standard. However, the slow convergence and enormous computational effort required by this scheme, make it frequently impractical. Consequently, recent scientific focus has shifted to a sampling-based multilevel Monte Carlo method (MLMC) that is computationally more suitable. Therefore, the objective of this research is to incorporate the multilevel Monte Carlo framework, where a novel method for determining the covariance of the stochastic solution via MLMC using h-statistics is presented.

%The statistical finite element method (statFEM) \cite{girolami_statistical_2021} which synthesizes finite element models with the observation data, performs Bayesian update on the stochastic FEM solution instead---of conventional way---on the model parameters of the physics-based governing equations. The framework consists of two vital stages of problem solving i.e. the forward and the inverse formulation. 
%Confining to the former, it is well known that solving stochastic differential equations with high-dimensional random parameters--with the so-called curse of dimensionality issue---is a major challenge in uncertainty quantification (UQ). In order to solve such stochastic problems, the Monte Carlo method (MC) has long been considered the gold standard. However, the slow convergence and enormous computational effort required by this scheme, make it frequently impractical. Consequently, recent scientific focus has shifted to a sampling-based multilevel Monte Carlo method (MLMC) that is computationally more suitable.
%%, especially in high-dimensional random field/process scenario.
%Therefore, the objective of this research is to incorporate the multilevel Monte Carlo framework into the statFEM forward problem, where a novel method for determining the covariance of the stochastic solution via MLMC using h-statistics is presented.

%\section{Novelty}



\section{State of the art}

 Most of the literature \cite{hoel_multilevel_2016,chernov_multilevel_2021} focus on estimation of covariance using multilevel Monte Carlo method in the context of ensemble Kalman filter or data assimilation to solve Bayesian inverse problems.
 Similarly, a new multifidelity ensemble Kalman filter algorithm building upon the theory of multivariate control variates, and on reduced order model data assimilation approaches is developed in \cite{popov_multifidelity_2020}.
% However, such control variate based multifidelity frameworks are out of scope of this work.
 On the other hand, the study \cite{mycek_multilevel_2019} estimate multilevel covariance for sensitivity analysis to derive a multilevel estimation of Sobol' indices, whose building blocks can be written as covariance terms in a pick-and-freeze formulation. 
%Kalman filtering, data assimilation \cite{hoel_multilevel_2016} The case of covariance has been addressed for the
%case of the covariance matrix used in the ensemble Kalman filter or data assimilation.
%; forecast covariance matrix must be computed to perform the analysis step of the ensemble Kalman filter (EnKF); sample covariances are required to compute solutions to inverse problems in ensemble Kalman inversion
The author in \cite{maurais_multifidelity_nodate} also proposes two other ways of estimating multifidelity covariance. The first method is about inducing the positive-definiteness property in the algorithm by construction; that is, by appplying linear control variates to sample covariance matrix logarithms, which are symmetric matrices residing in tangent spaces to the SPD manifold. This is called as the tangent space or log-linear control variate estimator. The other approach departs from the control variate formulation, and the multifidelity covariance estimator is defined as the solution to a regression problem on tangent spaces to product manifolds of SPD matrices.


%\section{Problem description}
%
%\subsection{Deterministic setting}
%
%%As a simple example of such an equation, the reader may think of the well known
%%thermal conduction equation
%
%Let be given a physical body defined on domain $\spatialdomain \subset \Euclideanspace $  in a $d-$ dimensional Euclidean space $\Euclideanspace$ (here $d = 2$ or $d = 3$). Steady state heat equation:
%
%\begin{equation}\label{Eq:deterministic-cond}
%	\begin{aligned}
%		-\nabla\cdot(\genSecTensor(\vek{x}) \nabla \uu(\vek{x})) &= \heatsource(\vek{x})\quad \forall \vek{x}\in\spatialdomain, \\
%		\uu(\vek{x}
%		) &= {\uu}_0,  \quad \forall \vek{x}
%		\in \Gamma_D, \\
%		\genSecTensor(\vek{x}) \nabla \uu(\vek{x})\cdot\vek{n}(\vek{x}) &= {g}(\vek{x}), \quad \forall \vek{x} \in \Gamma_N,
%	\end{aligned}
%\end{equation}
%where $\genSecTensor(\vek{x})$ represents thermal conductivity tensor, belonging to a space of open convex cone of d-dimensional real-valued second-order symmetric positive-definite (SPD) tensors:
%\begin{equation}
%	\PosSymSecRankSpace:=\{ \genSecTensor\in (\Euclideanspace\otimes\Euclideanspace) \mid 
%	\genSecTensor=\genSecTensor^T, \,\vek{z}^T \genSecTensor  \vek{z}>\vek{0}, \forall 
%	\vek{z}\in\Euclideanspace\setminus\{\vek{0}\} \}.
%\end{equation}
%Weak formulation:
%\begin{equation}\label{Eq:Weakform}
%	a(\uu(\vek{x}),\testfunction(\vek{x})) = l(\testfunction(\vek{x})), \; \forall\testfunction\in \solspace
%\end{equation}
%in which,
%\begin{equation}\label{Eq:RHSa}
%	a(\uu(\vek{x}),\testfunction(\vek{x})) = \int_\spatialdomain \nabla\testfunction(\vek{x})^T \cdot \genSecTensor(\vek{x}) \cdot \nabla \uu(\vek{x}) \di\spatialdomain,
%\end{equation}
%and
%\begin{equation}\label{Eq:LHSb}
%	l(\testfunction(\vek{x}))=\int_{\spatialdomain}\heatsource(\vek{x})\testfunction(\vek{x}
%	) \di\spatialdomain+\int_{\Gamma_N}{g}(\vek{x}
%	)\testfunction(\vek{x}
%	)\di \Gamma.
%\end{equation}
%Finite element approximation:
%\begin{equation}\label{Eq:u_approx}
%	\uu(\vek{x})\approx\uh(\vek{x}) = \sum_{j=1}^\nodes \solcoeff_j \shapefunc_j(\vek{x}).
%\end{equation}
%The weak form rewrites to
%\begin{equation}\label{Eq:Weak_form_approx}
%	a(\uh(\vek{x}),\testfunction_h(\vek{x})) = l(\testfunction_h(\vek{x})), \; \forall\testfunction_h\in \finitespace.
%\end{equation}
%After performing Galerkin projection of the residual, one may obtain a linear system of equations:
%\begin{equation}\label{Eq:lineareq}
%	\stiffnessmatrix\solvect=\vek{b},
%\end{equation}
%where
%\begin{equation}
%	\stiffnessmatrix = [\stiffnessmatrixele_{ij}],\  \stiffnessmatrixele_{ij} = \int_\spatialdomain \nabla \shapefunc_i(\vek{x})^T \cdot \genSecTensor(\vek{x}) \cdot \nabla \shapefunc_j(\vek{x}) \di\spatialdomain,
%\end{equation}
%and
%\begin{equation}
%	\vek{b}=[b_i],\ b_i=  \int_{\spatialdomain}\heatsource(\vek{x})\shapefunc_i(\vek{x}
%	) \di\spatialdomain+\int_{\Gamma_N}{g}(\vek{x}
%	)\shapefunc_i(\vek{x}
%	)\di \Gamma.
%\end{equation}
%
%\subsection{Uncertainty modelling: Gaussian Markov random field}
%
%Assuming that $\genSecTensor(\vek{x})$  represents an isotropic material, $\genSecTensor(\vek{x}) = \scalar(\vek{x}) \diag(\identitymatrix)$ is a diagonal matrix, where $\scalar(\vek{x})>0$ is a positive-definite scalar term. To incorporate the material uncertainty in spatial sense, the coefficient $\genSecTensor(\vek{x})$ is modelled as a tensor-valued SPD random field
%\begin{equation}\label{Eq:Tmapping}
%	\genSecTensor(\vek{x}, \event): \spatialdomain \times \samplespace\rightarrow\PosSymSecRankSpace
%\end{equation}
%on a probability space $(\samplespace,\sigmaalgebra,\probability)$. In other words, one may model
%\begin{equation}\label{Eq:scalar,odel}
%	\scalar(\vek{x}, \event): \spatialdomain \times \samplespace \rightarrow \mathbb{R}^+.
%\end{equation}
%Instead of modelling the previous equation, $\log(\scalar(\vek{x}, \event))$ can be modelled on $\mathbb{R}$ and take its exponential. Consequently, \feq{Eq:Tmapping} changes to:
%\begin{equation}\label{Eq:Tmapping}
%	\log(\genSecTensor(\vek{x}, \event)): \spatialdomain \times \samplespace\rightarrow\SymSecRankSpace,
%\end{equation}
%and taking $\exp(\log(\genSecTensor(\vek{x}, \event))) = \genSecTensor(\vek{x}, \event)$.
%In this work, $\log(\scalar(\vek{x}, \event)):=\logscalar(\vek{x}, \event) $ from \feq{Eq:scalar,odel} is modelled as a Gaussian Markov random field (GMRF) with Mat\'{e}rn covariance structure \cite{lindgren_explicit_2011, bulthuis_implementation_2022} which can be attained as a solution to a stochastic PDE of the form:
%\begin{equation}
%	(\kappa-\Delta)^{\alpha/2} \logscalar(\vek{x}, \event) = \mathcal{W}(\vek{x}, \event).
%\end{equation}
%With an assumption of $\alpha=2$ and suitable boundary conditions (Neumann or Robin), one may peform spatial discretization using finite element method from  \feq{Eq:u_approx} as
%\begin{equation}\label{}
%	\logscalar(\vek{x}, \event)\approx\logscalar_h(\vek{x}, \event) = \sum_{j=1}^\nodes \logscalar_j(\event) \shapefunc_j(\vek{x}).
%\end{equation}
%%, where $\samplespace$ 
%%represents the sample space containing all outcomes $\event\in\samplespace$, $\sigmaalgebra$ is the 
%%$\sigma$-algebra of measurable subsets of $\samplespace$, and $\probability$ is 
%%a probability measure.
%One has to basically solve the linear system of equations
%\begin{equation}\label{Eq:linGMRF}
%	\vek{K} \vek{L}(\event) = \vek{M}^{1/2} \vek{\xi}(\event)
%\end{equation}
%to obtain the GMRF realisations of $\scalar(\vek{x}, \event)$. Here, solution vector is
%$\vek{L}(\event) = [\zeta_j(\event)] \in \mathbb{R}^\nodes$ and the vector of independent standard Gaussian random variables is $\vek{\xi}(\event) = [\xi_j\sim\mathcal{N}(0, 1)] \in \mathbb{R}^\nodes$.  Furthermore, the entries of the matrices in the previous equation are given as:
%\begin{equation}
%	\begin{aligned}
%		{M_{ij}} &= \langle \shapefunc_i, \shapefunc_j \rangle\\
%		{G_{ij}} &= \langle \nabla \shapefunc_i, \nabla \shapefunc_j \rangle\\
%		K_{ij} &= \kappa^2 M_{ij} + G_{ij}
%	\end{aligned}
%\end{equation}
%To make $\vek{M}^{1/2} $ sparse in \feq{Eq:linGMRF}, the mass matrix $\vek{M}$ is approximated by a diagonal matrix of the form:
%\begin{equation}
%	\tilde{M_{ij}} =  \langle \shapefunc_i, 1 \rangle.
%\end{equation}
%
\section{Stochastic setting of the problem}

Let's consider, for instance, stochastic Poisson equation
\begin{equation}\label{Eq:stochastic-thm}
	\begin{aligned}
		-\nabla\cdot(\genSecTensor(\vek{x}, \event) \nabla \uu(\vek{x},\event)) &= \heatsource(\vek{x})\quad \forall \vek{x}\in\spatialdomain, \event\in\samplespace, \\
		\uu(\vek{x},\event)) &= {\uu}_0,  \quad \forall \vek{x}
		\in \Gamma_D, \\
		\genSecTensor(\vek{x}, \event) \nabla \uu(\vek{x},\event))\cdot\vek{n}(\vek{x}) &= {g}(\vek{x}), \quad \forall \vek{x} \in \Gamma_N,
	\end{aligned}
\end{equation}
where, only the diffusion coefficient $\genSecTensor$ is modelled as a random field
\begin{equation}\label{Eq:Tmapping}
	\genSecTensor(\vek{x}, \event): \spatialdomain \times \samplespace\rightarrow\PosSymSecRankSpace.
\end{equation}
%Weak formulation under uncertainty:
%\begin{equation}\label{Eq:Sto_Weakform}
%	a(\uu(\vek{x},\event),\testfunction(\vek{x},\event)) = l(\testfunction(\vek{x},\event)), \; \forall\testfunction(\vek{x},\event) \in \solspace\otimes \stospace,
%\end{equation}
After performing weak formulation, the stochastic finite element solution reads
\begin{equation}\label{Eq:Sto_u_approx}
	\uh(\vek{x},\event) = \sum_{j=1}^{\nodes} \solcoeff^h_j(\event) \shapefunc_j(\vek{x}).
\end{equation}
Consequently, one obtains linear system of equations
\begin{equation}\label{}
	\stiffnessmatrix(\event)\solvect^h(\event)=\vek{b},
\end{equation}
in which, $\solvect^h(\event) = [u^h_1(\event), u^h_2(\event),....,u^h_M(\event)]^T  \in \mathbb{R}^\nodes $ is the stochastic nodal solution vector.  
%with
%\begin{equation}
%	\stiffnessmatrix(\event) = [\stiffnessmatrixele_{ij}(\event)],\  \stiffnessmatrixele_{ij}(\event) = \int_\spatialdomain \nabla \shapefunc_i(\vek{x})^T \cdot \genSecTensor(\vek{x}, \event) \cdot \nabla \shapefunc_j(\vek{x}) \di\spatialdomain,
%\end{equation}
%
%%\section{MLMC covariance estimator}
%
%\section{Uncertainty propagation: multilevel Monte Carlo method}
%
%%Let $\left\lbrace \meshlevel=0,1,2...,\LL \right\rbrace$ be a generalised increasing sequence---in the context of decreasing the element size $h$---of nested mesh-grids $\mathcal{T}_\meshlevel$, a regular (non-degenerate) partition of  the computational domain $\mathcal{G}$ of the problem described. Here $\meshlevel$ denotes the mesh level, and $\LL$ represents the finest mesh. Due to the linearity of the expectation operator, one may express the \acrshort{mlmc} (also denoted by ML) mean estimate of the mean $\mumu(\uhL)$ using a set of samples $\left\lbrace \Nl \right\rbrace:=\left\lbrace \N_0,\N_1,...,\N_L \right\rbrace$ as \cite{Heinrich2001}
%
%\subsection{Multilevel Monte Carlo (MLMC) mean estimator}
%
%MLMC mean \cite{Heinrich2001,Cliffe2011}:
%
%\begin{eqnarray}\label{Eq:meanMLMC}
%	\muML(\uhLNL) &:=& \mu^{\text{MC}}(\uhONO) + \sum_{\meshlevel=1}^{\numofmesh}  \mu^{\text{MC}}(\uhlNl - \uhllNl) \nonumber\\
%	&=& \sum_{\meshlevel=0}^{\numofmesh} \mu^{\text{MC}}(\YhlNl).
%\end{eqnarray}
%%Here $\mu^{\text{MC}}(\uhONO)$ is the \acrshort{mc} estimator of mean $\mu(\uhO)$ on level $l=0$ using $N_0$ samples, and $\mu^{\text{MC}}(\uhlNl - \uhllNl)$ represents the approximation of mean $\mu(\uhlNl - \uhllNl)$ with $\meshlevel>0$ and $\Nl$ samples; $\mu^{\text{MC}}(\YhlNl)$ is the \acrshort{mc} estimator of $\mu(\Yhl)$ such that for $l=0$, $\YhONO = \uhONO$, otherwise $\YhlNl:=\uhlNl -\uhllNl$. Note that each term $\YhlNl, \ \meshlevel\ge{0}$ is sampled independently, whereas for $l>0$ the quantities $\uhlNl$ and $\uhllNl$ in $Y_{h_l,\Nl}$ are considered to be strongly correlated.
%
%Mean square error(MSE) of MLMC mean estimator:
%
%\begin{equation}\label{Eq:MLMCerror1}
%	{\eeML_{\text{MSE}}}(\muML) = \sum_{\meshlevel=0}^{\numofmesh} \frac{\var(\Yhl)}{\Nl}+(\mathbb{E}(\uhL)-\mathbb{E}(\uu))^2.
%\end{equation}
%
%Total computational cost of MLMC mean estimator:
%
%\begin{equation}
%	\mathcal{C}(\muML):=\sum_{\meshlevel=0}^{\LL}\Nl\costlevel
%\end{equation}
%
%Constrained optimization problem to determine the number of samples in each mesh-level:
%
%\begin{equation}\label{Eq:costfn}
%	\costfunction = \text{arg} \min\limits_{\optSam}  \sum_{\meshlevel=0}^{\LL} \left( \optSam\costlevel +  \Lagrange \frac{\mathbb{V}\text{ar}(\YhlNl)}{\Nl}\right)
%\end{equation} 	
%
%%\subsection{Multilevel Monte Carlo (MLMC) variance estimator}
%%
%%\cite{krumscheid_quantifying_2020,bierig_convergence_2015}

\section{Classical Monte Carlo estimation of covariance}
The goal is to determine the covariance of random vector  $\solvect^h(\event)$:
\begin{equation}\label{Eq:cov_analytical1}
	\cov(\solvect^h, \solvect^h) :=  \mathbb{E}((\solvect^h - \mathbb{E}(\solvect^h)) (\solvect^h - \mathbb{E}(\solvect^h))^T),
\end{equation}
which takes values in the open convex cone of $\nodes$-dimensional real-valued second-order positive-definite tensors/matrices
\begin{equation}\label{Eq:PosSymSpace}
	\PosSymMatSpace(\nodes):=\{ \genSecTensor\in (\mathbb{R}^\nodes\otimes\mathbb{R}^\nodes) \mid 
	\genSecTensor=\genSecTensor^T, \,\vek{z}^T \genSecTensor  \vek{z}>\vek{0}, \forall 
	\vek{z}\in\mathbb{R}^\nodes\setminus\vek{0} \}.
\end{equation}
Alternatively, one may also define the $(i, j)$ entry of the covariance matrix $\cov(\solvect^h, \solvect^h)$ from \feq{Eq:cov_analytical1} as
\begin{equation}\label{Eq:cov_analytical}
	\cov(u^h_i, u^h_j) = \mathbb{E}((u^h_i - \mathbb{E}(u^h_i)) (u^h_j - \mathbb{E}(u^h_j))),
\end{equation}
the nomenclature of which for simplicity will be adopted in the rest of the work.
In the previous equation, the expectation operator $\mathbb{E}$ of a scalar-valued function, let's say of a random variable $Y(\event):\samplespace \rightarrow \mathbb{R} $, is defined analytically in the form
\begin{equation}
	\mathbb{E}(Y(\event)) = \mu(Y(\event))  = \int_{\samplespace} Y(\event) \mathbb{P}(\textrm d\event).
\end{equation}
Here $Y$ maybe denoted by $u^h_i$ or $u^h_j$ from \feq{Eq:cov_analytical}.
Due to the difficulty in performing such analytical integration in the previous equation, one may obtain an estimate of the mean using MC procedure:
\begin{equation}
	\mu(Y)  \approx \muMC(Y) = \frac{1}{N} \sum_{k=1}^{N} Y(\event_k).
\end{equation}
Therefore, the estimation of covariance in \feq{Eq:cov_analytical} by MC transforms to
\begin{equation}\label{Eq:cov_sample}
	\covMC(u^h_i, u^h_j) = \muMC((u^h_i - \muMC(u^h_i)) (u^h_j - \muMC(u^h_j))).
\end{equation}
Following this, the \acrfull{mse} of covariance estimator is given as
\begin{equation}
	\textrm{MSE}(\covMC) = 	\var(\covMC(u^h_i, u^h_j)) + (\cov(u^h_i, u^h_j) - \cov(u_i, u_j))^2,
\end{equation}
with the assumption that $\covMC(u^h_i, u^h_j)$ is an unbiased estimator, meaning that $\mathbb{E}(\covMC(u^h_i, u^h_j)) = \cov(u^h_i, u^h_j)$. Note that, in the previous equation, the first terms signifies the sampling/stochastic accuracy, whereas, the second term represents the error due to deterministic discretization, i.e.
\begin{equation}\label{Eq:varMCcov}
	\var(\covMC(u^h_i, u^h_j)) = \frac{\mu_{2,2}(u^h_i, u^h_j)}{\N} - \frac{(\N-2)\cov(u^h_i, u^h_j)^2}{\N(\N-1)}+\frac{\var(u^h_i) \var(u^h_j)}{\N(\N-1)}, 
\end{equation}
where
\begin{equation}
	\mu_{r,s}(u^h_i, u^h_j) =  \mathbb{E}((u^h_i - \mathbb{E}(u^h_i))^r (u^h_j - \mathbb{E}(u^h_j))^s), 
\end{equation}
represents the bivariate central moment with $r,s \ge 0$.  
%$\mu_{1,1}(u^h_i, u^h_j) = \cov(u^h_i, u^h_j)$ is the covariance and $\mu_{0,2}(u^h_i, u^h_j) = \var(u^h_j)$ denotes the variance of random variable $u^h_j$.

The challenge is to obtain an unbiased estimation (of possibly also minimum variance) of sampling error in \feq{Eq:varMCcov}. In this regard, \cite{mycek_multilevel_2019} reports only the satisfaction of upper bounds of such an error estimate, i.e.
\begin{equation}\label{Eq:upperboud_MC}
	\var(\covMC(u^h_i, u^h_j)) \le \frac{1}{\N-1} \sqrt{\mu_{4}(u^h_i) \mu_{4}(u^h_j)},
\end{equation}
where $\mu_{4}(u^h_i) = \mathbb{E} ((u^h_i - \mathbb{E}(u^h_i))^4) $ is the fourth order central moment.

\section{Monte Carlo estimation of covariance using h-statistics}
Rewriting the estimation of covariance in \feq{Eq:cov_sample} using h-statistics \cite{Colin_Rose:2002} as 
\begin{equation}\label{Eq:h11}
\covMC(u^h_i, u^h_j) = \h_{1,1}(u^h_i, u^h_j)=	\frac{\N s_{1,1}-s_{0,1} s_{1,0}}{(\N-1) \N},
\end{equation}
where, the bivariate power sum,
\begin{equation}
	s_{a,b}(u^h_i, u^h_j) = \sum_{k=1}^{\N} u^h_i(\event_k)^a u^h_j(\event_k)^b.
\end{equation}
Similarly, the \feq{Eq:varMCcov} can be re-expressed in the form of bivariate central moments:
\begin{equation}\label{Eq:varMCcovmu}
	\var(\h_{1,1}(u^h_i, u^h_j)) = \frac{\mu_{2,2}(u^h_i, u^h_j)}{\N} - \frac{(\N-2)\mu_{1,1}(u^h_i, u^h_j)^2}{\N(\N-1)}+\frac{\mu_{0,2}(u^h_i, u^h_j) \mu_{2,0}(u^h_i, u^h_j)}{\N(\N-1)}, 
\end{equation}
in which, $\mu_{1,1}(u^h_i, u^h_j) = \cov(u^h_i, u^h_j)$ is the covariance and $\mu_{0,2}(u^h_i, u^h_j) = \var(u^h_j)$ denotes the variance of random variable $u^h_j$.

By replacing the bivariate central moments in the previous equation by h-statistics 
%\begin{equation}\label{Eq:varMCcovh2}
%		\varMC(\covMC) = \frac{\h_{2,2}(u^h_i, u^h_j)}{\N} - \frac{(\N-2)\h_{1,1}(u^h_i, u^h_j)^2}{\N(\N-1)}+\frac{\h_{0,2}(u^h_i, u^h_j) \h_{2,0}(u^h_i, u^h_j)}{\N(\N-1)}, 
%\end{equation}
one does not directly obtain an unbiased estimate due to the inherent non-linear transformation of statistics. 
Therefore, similar to the approach mentioned in \cite{krumscheid_quantifying_2020}, let's consider an ansatz of the form
\begin{equation}\label{Eq:varMCcovh21}
	\varMC(\h_{1,1}) = {\aone \h_{2,2}(u^h_i, u^h_j)} + {\atwo \h_{1,1}(u^h_i, u^h_j)^2 + \athree \h_{0,2}(u^h_i, u^h_j) \h_{2,0}(u^h_i, u^h_j)},
\end{equation}
where $\h_{1,1} = \covMC$ is the sample covariance in h-statistics form of \feq{Eq:cov_sample}.
Here, to attain an unbiased estimator $\varMC(\h_{1,1})$, the condition $\mathbb{E}(\varMC(\h_{1,1})) = \var(\h_{1,1})$ must hold. To this, the expectation of $\varMC(\h_{1,1})$ in terms of bivariate central moments is given---via mathStatica \cite{Colin_Rose:2002}---as
\begin{align}\label{Eq:varMCcovh22}
	\begin{split}
		\mathbb{E}(\varMC(\h_{1,1})) =& \frac{(\aone\N+\atwo+\athree) \mu_{2,2}}{\N} + \frac{(2 \athree + \atwo (2 - 2 \N + 				
																\N^2)){\mu_{1,1}}^2}{\N(\N-1)}+ \\ 
															 &	\frac{(\atwo + \athree (-1 + \N)^2)\mu_{0,2} \mu_{2,0}}{\N(\N-1)}.
	\end{split}
\end{align}
By comparing the above equation with \feq{Eq:varMCcovmu} and solving a linear system of equations, the values of constants can be determined as $\aone = \frac{\N-1}{3-2\N+\N^2}$, $\atwo = \frac{-5+4\N-\N^2}{-6+7\N-4\N^2+\N^3}$ and $\athree=\frac{\N-1}{-6+7\N-4\N^2+\N^3}$.
Finally, the unbiased closed form expression of $\varMC(\h_{1,1})$ (as compared to only the upper bound in \feq{Eq:upperboud_MC}) in \feq{Eq:varMCcovh21} can be obtained in the form of power sums as
\begin{align}
	\begin{split}
	\varMC(\h_{1,1})  = & \frac{1}{(\N-3) (\N-2) (\N-1)^2 \N^2} \left( \N \left(\left(-\N^2+\N+2\right) s_{1,1}^2+ \right. \right. \\
									 & \left. \left. (\N-1)^2 \left(\N s_{2,2}-2 s_{1,0} s_{1,2}\right)+ (\N-1) s_{0,2} \left(s_{1,0}^2-s_{2,0}\right)\right)+ \right. \\ 
									 & \left.  s_{0,1}^2 \left((6-4 \N) s_{1,0}^2+(\N-1) \N s_{2,0}\right)  \right. \\
									 &  \left.   -2 \N s_{0,1} \left((\N-1)^2 s_{2,1}+(5-3 \N) s_{1,0} s_{1,1}\right)\right).
	\end{split}
\end{align}

\section{Classical multilevel Monte Carlo (MLMC) covariance estimator}

The multilevel Monte Carlo covariance estimator is 
\begin{equation}\label{Eq:covMLMC}
\covML(u^{h_L}_i, u^{h_L}_j) := \cov^{\text{MC}}(u^{h_0}_i, u^{h_0}_j) + \sum_{\meshlevel=1}^{\numofmesh}  \cov^{\text{MC}}(u^{h_l}_i, u^{h_l}_j) - \cov^{\text{MC}}(u^{h_{l-1}}_i, u^{h_{l-1}}_j).
\end{equation}
For simplicity, let's introduce:
\begin{equation}\label{Eq:Zl}
	\Zl= 
	\begin{cases}
		\covMC(u^{h_0}_i, u^{h_0}_j),\quad &\meshlevel=0,\\
		\covMC(u^{h_l}_i, u^{h_l}_j) - \covMC(u^{h_{l-1}}_i, u^{h_{l-1}}_j),\quad &\meshlevel>0.
	\end{cases}
\end{equation}
Therefore, \feq{Eq:covMLMC} transforms to
\begin{equation}\label{Eq:sumZl}
	\covML	= \sum_{\meshlevel=0}^{\numofmesh} \Zl.
\end{equation}
A multilevel covariance estimator from \feq{Eq:covMLMC} has the drawback that it cannot ensure the covariance matrices' positive-definiteness property, which is outlined in \feq{Eq:PosSymSpace}. This is because subtracting one positive-definite matrix from another does not guarantee that the resulting matrix is positive-definite---which is vital for the stability of the algorithm \cite{hoel_multilevel_2016,maurais_multifidelity_nodate}.
%The downside of a multilevel covariance estimator in \feq{Eq:covMLMC} is its inability to guarantee the positive-definiteness property of covariance matrices as described in \feq{Eq:PosSymSpace}. This is due to the fact that subtraction of one positive-definite matrix from another does not ensure positive-definiteness of the resulting matrix.
To overcome this drawback, the authors in  \cite{hoel_multilevel_2016} impose the positive-definiteness by performing eigen-decomposition of $\covML(u^{h_L}_i, u^{h_L}_j)$
\begin{equation}
	\covML = \sum_{i=1}^{\nodes} \lambda_i \vek{q}_i \vek{q}_i^T,
\end{equation}
such that, the negative-valued eigenvalues
\begin{equation}
	\widetilde{\cov}^{\textrm{ML}}  = \sum_{i=1;\lambda_i>0}^{\nodes} \lambda_i \vek{q}_i \vek{q}_i^T,
\end{equation}
are removed. Other computationally cheaper techniques such as banding, shrinkage, threshold and so on can also be considered as alternatives to spectral decomposition. 

The \acrshort{mse} of MLMC covariance estimator reads
\begin{equation}\label{Eq:MSEcovML}
	\textrm{MSE}(\covML)  =  \var(\covML) + (\cov(u^{h_L}_i, u^{h_L}_j) - \cov(u_i, u_j))^2
\end{equation}
in which the upper bound of the sampling error (the first term in the above equation) can be derived as \cite{mycek_multilevel_2019}
\begin{align}
	\begin{split}
		\var(\covML)  =& \sum_{\meshlevel=0}^{\numofmesh} \var(\Zl) \le \frac{1}{2} \sum_{\meshlevel=0}^{\numofmesh} \frac{1}{\Nl-1} \left( 
									\sqrt{\mu_{4}(\text{X}^-(u^{h_l}_i))\mu_{4}(\text{X}^+(u^{h_l}_j))} + \right. \\
								  & \left. \sqrt{\mu_{4}(\text{X}^+(u^{h_l}_i))\mu_{4}(\text{X}^-(u^{h_l}_j))} \right).
	\end{split}
\end{align}
Here $\text{X}^+(u^{h_l}_i) = u^{h_l}_i + u^{h_{l-1}}_i$  and $\text{X}^-(u^{h_l}_i) = u^{h_l}_i - u^{h_{l-1}}_i$.

\section{Multilevel Monte Carlo (MLMC) covariance estimator using h-statistics}

The multilevel Monte Carlo covariance estimator in h-statistics is 
\begin{equation}\label{Eq:covMLMChstat}
	\h_{1,1}^{\text{ML}}(u^{h_L}_i, u^{h_L}_j) :=\h_{1,1}(u^{h_0}_i, u^{h_0}_j) + \sum_{\meshlevel=1}^{\numofmesh}  \h_{1,1}(u^{h_l}_i, u^{h_l}_j) - \h_{1,1}(u^{h_{l-1}}_i, u^{h_{l-1}}_j).
\end{equation}
As the second part of the above equation is made up of four variables $(u^{h_l}_i, u^{h_l}_j, u^{h_{l-1}}_i, u^{h_{l-1}}_j)$, therefore, one may rewrite it in the form of quadrivariate h-statistic:
\begin{align}\label{Eq:covMLMChstat1}
	\begin{split}
		\h_{1,1}^{\text{ML}}(u^{h_L}_i, u^{h_L}_j) =&  \h_{1,1}(u^{h_0}_i, u^{h_0}_j) + \sum_{\meshlevel=1}^{\numofmesh}  \h_{1,1,0,0}(u^{h_l}_i, u^{h_l}_j,u^{h_{l-1}}_i, u^{h_{l-1}}_j) - \\
																				  & \h_{0,0,1,1}(u^{h_l}_i, u^{h_l}_j,u^{h_{l-1}}_i, u^{h_{l-1}}_j).
	\end{split}
\end{align}
Subsequently, \feq{Eq:Zl} rewrites to
\begin{equation}\label{Eq:Zl}
	\Zl= 
	\begin{cases}
		\h_{1,1}(u^{h_0}_i, u^{h_0}_j),\quad &\meshlevel=0,\\
		\h_{1,1,0,0}(u^{h_l}_i, u^{h_l}_j,u^{h_{l-1}}_i, u^{h_{l-1}}_j) - \h_{0,0,1,1}(u^{h_l}_i, u^{h_l}_j,u^{h_{l-1}}_i, u^{h_{l-1}}_j),\quad &\meshlevel>0,
	\end{cases}
\end{equation}
and, similarly, \feq{Eq:sumZl} to
\begin{equation}
	\h_{1,1}^{\text{ML}}	= \sum_{\meshlevel=0}^{\numofmesh} \Zl.
\end{equation}

For $\meshlevel=0$, $Z_0 = \h_{1,1}$ is described similarly as shown in \feq{Eq:h11}, and when $\meshlevel>0$,
\begin{equation}
	\Zl = \frac{\Nl s_{1,1,0,0}-s_{0,1,0,0} s_{1,0,0,0}}{(\Nl-1) \Nl}-\frac{\Nl s_{0,0,1,1}-s_{0,0,0,1} s_{0,0,1,0}}{(\Nl-1) \Nl}.
\end{equation}
Here, the quadrivariate power sum, for each $\ml$, is given as 
\begin{equation}
	s_{a,b,c,d}(u^{h_l}_i, u^{h_l}_j,u^{h_{l-1}}_i, u^{h_{l-1}}_j) = \sum_{k=1}^{\N} u^{h_l}_i(\event_k)^a u^{h_l}_j(\event_k)^b u^{h_{l-1}}_i(\event_k)^c u^{h_{l-1}}_j(\event_k)^d.
\end{equation}

The MSE of MLMC covariance in \feq{Eq:MSEcovML} is
\begin{equation}
	\textrm{MSE}(\h_{1,1}^{\text{ML}})  =  \var(\h_{1,1}^{\text{ML}}) + (\cov(u^{h_L}_i, u^{h_L}_j) - \cov(u_i, u_j))^2.
\end{equation}
Here, the first part, which is the statistical error, is expressed as 
\begin{equation}
	\var(\h_{1,1}^{\text{ML}})	= \sum_{\meshlevel=0}^{\numofmesh} \var(\Zl).
\end{equation}
Furthermore, $\var(Z_0)$ is determined as given in \feq{Eq:varMCcovmu}, however, for $\ml>0$, the variance of $\Zl$ is written in the form of quadrivariate central moments:
\begin{align}\label{Eq:varZl}
	\begin{split}
		\var(\Zl) =& -\frac{(\Nl-2) \mu _{0,0,1,1}^2}{(\Nl-1) \Nl}+\frac{2 \mu _{1,1,0,0} \mu _{0,0,1,1}}{\Nl}+\frac{\mu _{0,0,0,2} \mu _{0,0,2,0}}{(\Nl-1) \Nl}+\frac{\mu _{0,0,2,2}}{\Nl}+ \\
						& \frac{\mu _{0,2,0,0} \mu _{2,0,0,0}}{(\Nl-1) \Nl}+\frac{\mu _{2,2,0,0}}{\Nl}-\frac{2 \mu _{1,1,1,1}}{\Nl}-\frac{(\Nl-2) \mu _{1,1,0,0}^2}{(\Nl-1) \Nl}- \\
						& \frac{2 \mu _{0,1,1,0} \mu _{1,0,0,1}}{(\Nl-1) \Nl}-\frac{2 \mu _{0,1,0,1} \mu _{1,0,1,0}}{(\Nl-1) \Nl}.
	\end{split}
\end{align}
Here, by setting $(u^{h_l}_i, u^{h_l}_j,u^{h_{l-1}}_i, u^{h_{l-1}}_j) \equiv (G,H,I,J) $ for each $\ml$, the multivariate central moment is defined as 
\begin{equation}
	\mu_{p,q,r,s}(G,H,I,J) =  \mathbb{E}((G- \mathbb{E}(G))^p (H - \mathbb{E}(H))^q (I - \mathbb{E}(I))^r (J - \mathbb{E}(J))^s).
\end{equation}
To obtain an unbiased estimate of $\var(\Zl)$ in \feq{Eq:varZl}, an Ansatz is assumed
\begin{align}\label{Eq:varMCZl}
	\begin{split}
		\varMC(\Zl) =& a_1 {h _{0,0,1,1}^2}+a_2{ h _{1,1,0,0} h _{0,0,1,1}}+ a_3 {h _{0,0,0,2} h _{0,0,2,0}}+ a_4 {h _{0,0,2,2}}+ \\
							   & a_5 {h _{0,2,0,0} h _{2,0,0,0}}+ a_6 {h _{2,2,0,0}}+ a_7 {h _{1,1,1,1}}+ a_8 {h _{1,1,0,0}^2}+ \\ 
							   & a_9 {h _{0,1,1,0} h _{1,0,0,1}}+ a_{10}{ h _{0,1,0,1} h _{1,0,1,0}}.
	\end{split}
\end{align}
Then, the expectation of above expression in quadrivariate central moments is determined using mathStatica \cite{Colin_Rose:2002} as
\begin{align}
	\begin{split}
		\mathbb{E}(\varMC(\Zl)) =& \frac{\mu _{0,0,2,2} (a_1+a_2+a_3 \Nl)}{\Nl}+ \frac{\mu _{0,0,1,1}^2 \left(a_1 \Nl^2-2 a_1 \Nl+2 a_1+2 a_2\right)}{(\Nl-1) \Nl}+ \\
													 & \frac{\mu _{0,0,0,2} \mu _{0,0,2,0} \left(a_1+a_2 \Nl^2-2 a_2 \Nl+a_2\right)}{(\Nl-1) \Nl}+ \frac{\mu _{2,2,0,0} (a_{10} \Nl+a_7+a_9)}{\Nl}+ \\
													 & \frac{\mu _{1,1,1,1} (a_4+a_5+a_6+a_8 \Nl)}{\Nl}+ \frac{\mu _{1,1,0,0} \mu _{0,0,1,1} \left(a_4+a_5+a_6 \Nl^2-2 a_6 \Nl+a_6\right)}{(\Nl-1) \Nl}+ \\
													 & \frac{\mu _{0,1,1,0} \mu _{1,0,0,1} \left(a_4 \Nl^2-2 a_4 \Nl+a_4+a_5+a_6\right)}{(\Nl-1) \Nl}+ \\
													 & \frac{\mu _{0,1,0,1} \mu _{1,0,1,0} \left(a_4+a_5 \Nl^2-2 a_5 \Nl+a_5+a_6\right)}{(\Nl-1) \Nl}+ \\
													 & \frac{\mu _{1,1,0,0}^2 \left(a_7 \Nl^2-2 a_7 \Nl+2 a_7+2 a_9\right)}{(\Nl-1) \Nl}+ \\
													 & \frac{\mu _{0,2,0,0} \mu _{2,0,0,0} \left(a_7+a_9 \Nl^2-2 a_9 \Nl+a_9\right)}{(\Nl-1) \Nl}.
	\end{split}
\end{align}
Comparing the previous equation and \feq{Eq:varZl}, and subsequently solving the linear system of equations, the values of constants are given as, 
$ a_1=-\frac{\Nl^2-4 \Nl+5}{\Nl^3-4 \Nl^2+7 \Nl-6}$, $a_2=-\frac{1-\Nl}{\Nl^3-4 \Nl^2+7 \Nl-6}$ $a_3=-\frac{1-\Nl}{\Nl^2-2 \Nl+3}$, $a_4=-\frac{2 (\Nl-1)}{\Nl^3-4 \Nl^2+7 \Nl-6}$, $a_5=-\frac{2 (\Nl-1)}{\Nl^3-4 \Nl^2+7 \Nl-6}$, $a_6=\frac{2 \left(\Nl^2-3 \Nl+4\right)}{\Nl^3-4 \Nl^2+7 \Nl-6}$, $a_7=-\frac{\Nl^2-4 \Nl+5}{\Nl^3-4 \Nl^2+7 \Nl-6}$, $a_8 =-\frac{2 (\Nl-1)}{\Nl^2-2 \Nl+3}$, $a_9 =-\frac{1-\Nl}{\Nl^3-4 \Nl^2+7 \Nl-6}$ and $a_{10}=-\frac{1-\Nl}{\Nl^2-2 \Nl+3}$.

Substituting these values in \feq{Eq:varMCZl}, one finally gets the unbiased closed form expression:
\begin{align*}
%	\begin{split}
		\varMC(\Zl)=& \frac{1}{(\Nl-3) (\Nl-2) (\Nl-1)^2 \Nl^2} \\
							  & \left( s_{0,0,2,2} \Nl^4-2 s_{1,1,1,1} \Nl^4+ s_{2,2,0,0} \Nl^4-s_{0,0,1,1}^2 \Nl^3-s_{1,1,0,0}^2 \Nl^3-2 s_{0,0,1,0} s_{0,0,1,2} 		 
		                          \Nl^3- \right.\\
							  & \left. 2 s_{0,0,2,2} \Nl^3+ 2 s_{0,1,1,1} s_{1,0,0,0} \Nl^3+2 s_{0,1,0,0} s_{1,0,1,1} \Nl^3+ 2 s_{0,0,1,1} s_{1,1,0,0} \Nl^3+\right.\\
							  & \left. 2 s_{0,0,1,0} s_{1,1,0,1} \Nl^3+ 4 s_{1,1,1,1} \Nl^3-2 s_{1,0,0,0} s_{1,2,0,0} \Nl^3-2 s_{0,1,0,0} s_{2,1,0,0} \Nl^3-2 s_{2,2,0,0} \Nl^3+ \right.\\
							  & \left. s_{0,0,1,1}^2 \Nl^2+ s_{0,2,0,0} s_{1,0,0,0}^2 \Nl^2+s_{1,1,0,0}^2 \Nl^2+ 4 s_{0,0,1,0} s_{0,0,1,2} \Nl^2+ s_{0,0,2,2} \Nl^2-\right.\\
							  & \left. 4 s_{0,0,1,1} s_{0,1,0,0} s_{1,0,0,0} \Nl^2-2 s_{0,0,1,0} s_{0,1,0,1} s_{1,0,0,0} \Nl^2- 4 s_{0,1,1,1} s_{1,0,0,0} \Nl^2- \right. \tag{\stepcounter{equation}\theequation}\\
							  & \left. 2 s_{0,0,1,0} s_{0,1,0,0} s_{1,0,0,1} \Nl^2+ 2 s_{0,1,1,0} s_{1,0,0,1} \Nl^2+2 s_{0,1,0,1} s_{1,0,1,0} \Nl^2-4 s_{0,1,0,0} s_{1,0,1,1} \Nl^2-\right.\\ 
							  & \left. 4 s_{0,0,1,1} s_{1,1,0,0} \Nl^2+ 6 s_{0,1,0,0} s_{1,0,0,0} s_{1,1,0,0} \Nl^2-4 s_{0,0,1,0} s_{1,1,0,1} \Nl^2-2 s_{1,1,1,1} \Nl^2+\right.\\
							  & \left. 4 s_{1,0,0,0} s_{1,2,0,0} \Nl^2+s_{0,1,0,0}^2 s_{2,0,0,0} \Nl^2-s_{0,2,0,0} s_{2,0,0,0} \Nl^2+ 4 s_{0,1,0,0} s_{2,1,0,0} \Nl^2+ \right.\\
							  & \left. s_{2,2,0,0} \Nl^2+2 s_{0,0,1,1}^2 \Nl-4 s_{0,1,0,0}^2 s_{1,0,0,0}^2 \Nl-s_{0,2,0,0} s_{1,0,0,0}^2 \Nl+ \right.\\
							  & \left. 2 s_{1,1,0,0}^2 \Nl-2 s_{0,0,1,0} s_{0,0,1,2} \Nl+(\Nl-1) s_{0,0,0,2} \left(s_{0,0,1,0}^2-s_{0,0,2,0}\right) \Nl+ \right.\\
							  & \left. 8 s_{0,0,1,1} s_{0,1,0,0} s_{1,0,0,0} \Nl+2 s_{0,0,1,0} s_{0,1,0,1} s_{1,0,0,0} \Nl+ \right.\\
							  & \left. 2 s_{0,1,1,1} s_{1,0,0,0} \Nl+2 s_{0,0,1,0} s_{0,1,0,0} s_{1,0,0,1} \Nl-2 s_{0,1,1,0} s_{1,0,0,1} \Nl-2 s_{0,1,0,1} s_{1,0,1,0} \Nl+ \right.\\
							  & \left. 2 s_{0,1,0,0} s_{1,0,1,1} \Nl-2 s_{0,0,1,1} s_{1,1,0,0} \Nl-10 s_{0,1,0,0} s_{1,0,0,0} s_{1,1,0,0} \Nl+ \right.\\
							  & \left. 2 s_{0,0,1,0} s_{1,1,0,1} \Nl-2 s_{1,0,0,0} s_{1,2,0,0} \Nl-s_{0,1,0,0}^2 s_{2,0,0,0} \Nl+ \right.\\
							  & \left. s_{0,2,0,0} s_{2,0,0,0} \Nl-2 s_{0,1,0,0} s_{2,1,0,0} \Nl+6 s_{0,1,0,0}^2 s_{1,0,0,0}^2+ \right.\\
							  & \left. s_{0,0,0,1}^2 \left((6-4 \Nl) s_{0,0,1,0}^2+(\Nl-1) \Nl s_{0,0,2,0}\right)-2 s_{0,0,0,1} \right.\\
							  & \left. \left(s_{0,0,1,0} \left(\Nl (5-3 \Nl) s_{0,0,1,1}+2 (3-2 \Nl) s_{0,1,0,0} s_{1,0,0,0}+ 2 (\Nl-2) \Nl s_{1,1,0,0}\right)+ \right. \right.\\
							  & \left. \left. (\Nl-1) \Nl \left((\Nl-1) s_{0,0,2,1}+s_{0,1,1,0} s_{1,0,0,0}+s_{0,1,0,0} s_{1,0,1,0}-\Nl s_{1,1,1,0}+s_{1,1,1,0}\right)\right)\right)
%	\end{split}
\end{align*}

==> chapters/uncertainty_modelling.tex <==
%\subsection{Uncertainty modelling}
Assuming that $\genSecTensor(\vek{x})$  represents an isotropic material, $\genSecTensor(\vek{x}) = \scalar(\vek{x}) \diag(\identitymatrix)$ is a diagonal matrix, where $\scalar(\vek{x})>0$ is a positive-definite scalar term. To incorporate the material uncertainty in spatial sense, the coefficient $\genSecTensor(\vek{x})$ is modelled as a tensor-valued SPD random field
\begin{equation}\label{Eq:Tmapping}
	\genSecTensor(\vek{x}, \event): \spatialdomain \times \samplespace\rightarrow\PosSymSecRankSpace
\end{equation}
on a probability space $(\samplespace,\sigmaalgebra,\probability)$. In other words, one may model
\begin{equation}\label{Eq:scalar,odel}
	\scalar(\vek{x}, \event): \spatialdomain \times \samplespace \rightarrow \mathbb{R}^+.
\end{equation}
Instead of modelling the previous equation, $\log(\scalar(\vek{x}, \event))$ can be modelled on $\mathbb{R}$ and take its exponential. Consequently, \feq{Eq:Tmapping} changes to:
\begin{equation}\label{Eq:Tmapping}
	\log(\genSecTensor(\vek{x}, \event)): \spatialdomain \times \samplespace\rightarrow\SymSecRankSpace,
\end{equation}
and taking $\exp(\log(\genSecTensor(\vek{x}, \event))) = \genSecTensor(\vek{x}, \event)$.
%In this work, $\log(\scalar(\vek{x}, \event)):=\logscalar(\vek{x}, \event) $ from \feq{Eq:scalar,odel} is modelled as a Gaussian Markov random field (GMRF) with Mat\'{e}rn covariance structure \cite{lindgren_explicit_2011, bulthuis_implementation_2022} which can be attained as a solution to a stochastic PDE of the form:
%\begin{equation}
%	(\kappa-\Delta)^{\alpha/2} \logscalar(\vek{x}, \event) = \mathcal{W}(\vek{x}, \event).
%\end{equation}
%With an assumption of $\alpha=2$ and suitable boundary conditions (Neumann or Robin), one may peform spatial discretization using finite element method from  \feq{Eq:u_approx} as
%\begin{equation}\label{}
%	\logscalar(\vek{x}, \event)\approx\logscalar_h(\vek{x}, \event) = \sum_{j=1}^\nodes \logscalar_j(\event) \shapefunc_j(\vek{x}).
%\end{equation}
%%, where $\samplespace$ 
%%represents the sample space containing all outcomes $\event\in\samplespace$, $\sigmaalgebra$ is the 
%%$\sigma$-algebra of measurable subsets of $\samplespace$, and $\probability$ is 
%%a probability measure.
%One has to basically solve the linear system of equations
%\begin{equation}\label{Eq:linGMRF}
%	\vek{K} \vek{L}(\event) = \vek{M}^{1/2} \vek{\xi}(\event)
%\end{equation}
%to obtain the GMRF realisations of $\scalar(\vek{x}, \event)$. Here, solution vector is
%$\vek{L}(\event) = [\zeta_j(\event)] \in \mathbb{R}^\nodes$ and the vector of independent standard Gaussian random variables is $\vek{\xi}(\event) = [\xi_j\sim\mathcal{N}(0, 1)] \in \mathbb{R}^\nodes$.  Furthermore, the entries of the matrices in the previous equation are given as:
%\begin{equation}
%	\begin{aligned}
%		{M_{ij}} &= \langle \shapefunc_i, \shapefunc_j \rangle\\
%		{G_{ij}} &= \langle \nabla \shapefunc_i, \nabla \shapefunc_j \rangle\\
%		K_{ij} &= \kappa^2 M_{ij} + G_{ij}
%	\end{aligned}
%\end{equation}
%To make $\vek{M}^{1/2} $ sparse in \feq{Eq:linGMRF}, the mass matrix $\vek{M}$ is approximated by a diagonal matrix of the form:
%\begin{equation}
%	\tilde{M_{ij}} =  \langle \shapefunc_i, 1 \rangle.
%\end{equation}
